Investigations in Calabi-Yau modularity and mirror symmetry

This is the author's PhD thesis. Two main sections address various aspects of mirror symmetry for compact Calabi-Yau threefolds and the roles that classically modular varieties play in string theory compactifications. The main results include a study, and finding an application to the higher genus problem, of infinite Coxeter symmetries in the sets of Gopakumar-Vafa invariants; provision of a new class of solutions to the supersymmetric flux vacuum equations which have elsewhere been conjectured to give weight-two modular manifolds; provision of two new conjectural examples of weight-four modular varieties (rank-two attractors); and discussion of a set of numerical relations between infinite sums of Gromov-Witten invariants and critical L-values.

==> 6_36_genus0.tex <==
A ] B
{0, 0, 0, 0, 0, 1}]10
{0, 0, 0, 0, 1, 0}]12
{0, 0, 0, 0, 1, 1}]12
{0, 0, 0, 1, 1, 0}]1
{0, 0, 0, 1, 1, 1}]22
{0, 0, 0, 1, 1, 2}]1
{0, 0, 1, 1, 1, 1}]56
{0, 0, 1, 1, 1, 2}]56
{0, 0, 1, 1, 2, 1}]1
{0, 0, 1, 1, 2, 2}]22
{0, 0, 1, 1, 2, 3}]1
{0, 0, 1, 2, 2, 2}]12
{0, 0, 1, 2, 2, 3}]12
{0, 0, 2, 2, 2, 2}]10
{0, 0, 2, 2, 2, 3}]60
{0, 0, 2, 2, 2, 4}]10
{0, 0, 2, 2, 3, 3}]12
{0, 0, 2, 2, 3, 4}]12
{0, 0, 2, 3, 3, 3}]1
{0, 0, 2, 3, 3, 4}]22
{0, 0, 2, 3, 3, 5}]1
{0, 0, 3, 3, 3, 4}]56
{0, 0, 3, 3, 3, 5}]56
{0, 0, 3, 3, 4, 4}]1
{0, 0, 3, 3, 4, 5}]22
{0, 1, 1, 1, 1, 1}]174
{0, 1, 1, 1, 1, 2}]756
{0, 1, 1, 1, 1, 3}]174
{0, 1, 1, 1, 2, 1}]12
{0, 1, 1, 1, 2, 2}]540
{0, 1, 1, 1, 2, 3}]540
{0, 1, 1, 1, 2, 4}]12
{0, 1, 1, 1, 3, 1}]-2
{0, 1, 1, 1, 3, 2}]10
{0, 1, 1, 1, 3, 3}]96
{0, 1, 1, 1, 3, 4}]10
{0, 1, 1, 1, 3, 5}]-2
{0, 1, 1, 2, 2, 2}]474
{0, 1, 1, 2, 2, 3}]1852
{0, 1, 1, 2, 2, 4}]474
{0, 1, 1, 2, 3, 2}]12
{0, 1, 1, 2, 3, 3}]540
{0, 1, 1, 2, 3, 4}]540
{0, 1, 1, 2, 3, 5}]12
{0, 1, 1, 2, 4, 3}]1
{0, 1, 1, 2, 4, 4}]22
{0, 1, 1, 2, 4, 5}]1
{0, 1, 1, 3, 3, 3}]174
{0, 1, 1, 3, 3, 4}]756
{0, 1, 1, 3, 3, 5}]174
{0, 1, 1, 3, 4, 4}]56
{0, 1, 1, 3, 4, 5}]56
{0, 1, 1, 4, 4, 4}]1
{0, 1, 1, 4, 4, 5}]22
{0, 1, 2, 2, 2, 2}]540
{0, 1, 2, 2, 2, 3}]6708
{0, 1, 2, 2, 2, 4}]6708
{0, 1, 2, 2, 2, 5}]540
{0, 1, 2, 2, 3, 2}]22
{0, 1, 2, 2, 3, 3}]2796
{0, 1, 2, 2, 3, 4}]8860
{0, 1, 2, 2, 3, 5}]2796
{0, 1, 2, 2, 3, 6}]22
{0, 1, 2, 2, 4, 3}]56
{0, 1, 2, 2, 4, 4}]1344
{0, 1, 2, 2, 4, 5}]1344
{0, 1, 2, 2, 4, 6}]56
{0, 1, 2, 2, 5, 4}]1
{0, 1, 2, 2, 5, 5}]22
{0, 1, 2, 3, 3, 3}]1344
{0, 1, 2, 3, 3, 4}]13968
{0, 1, 2, 3, 3, 5}]13968
{0, 1, 2, 3, 3, 6}]1344
{0, 1, 2, 3, 4, 3}]22
{0, 1, 2, 3, 4, 4}]2796
{0, 1, 2, 3, 4, 5}]8860
{0, 1, 2, 3, 5, 4}]12
{0, 1, 2, 4, 4, 4}]540
{0, 1, 3, 3, 3, 3}]798
{0, 1, 3, 3, 3, 4}]25662
{0, 1, 3, 3, 3, 5}]69528
{0, 1, 3, 3, 4, 3}]12
{0, 1, 3, 3, 4, 4}]6708
{0, 2, 2, 2, 2, 2}]756
{0, 2, 2, 2, 2, 3}]25662
{0, 2, 2, 2, 2, 4}]69516
{0, 2, 2, 2, 2, 5}]25662
{0, 2, 2, 2, 2, 6}]756
{0, 2, 2, 2, 3, 2}]56
{0, 2, 2, 2, 3, 3}]13968
{0, 2, 2, 2, 3, 4}]103000
{0, 2, 2, 2, 3, 5}]103000
{0, 2, 2, 2, 3, 6}]13968
{0, 2, 2, 2, 4, 3}]756
{0, 2, 2, 2, 4, 4}]25662
{0, 2, 2, 2, 4, 5}]69516
{0, 2, 2, 2, 5, 4}]540
{0, 2, 2, 3, 3, 2}]1
{0, 2, 2, 3, 3, 3}]8860
{0, 2, 2, 3, 3, 4}]176251
{0, 2, 2, 3, 3, 5}]425712
{0, 2, 2, 3, 4, 3}]540
{0, 2, 2, 3, 4, 4}]54504
{0, 2, 2, 4, 4, 3}]10
{0, 2, 3, 3, 3, 3}]6708
{0, 2, 3, 3, 3, 4}]342924
{0, 2, 3, 3, 4, 3}]474
{0, 3, 3, 3, 3, 3}]6204
{1, 1, 1, 1, 1, 1}]700
{1, 1, 1, 1, 1, 2}]8900
{1, 1, 1, 1, 1, 3}]8900
{1, 1, 1, 1, 1, 4}]700
{1, 1, 1, 1, 2, 1}]66
{1, 1, 1, 1, 2, 2}]8892
{1, 1, 1, 1, 2, 3}]27492
{1, 1, 1, 1, 2, 4}]8892
{1, 1, 1, 1, 2, 5}]66
{1, 1, 1, 1, 3, 1}]-24
{1, 1, 1, 1, 3, 2}]180
{1, 1, 1, 1, 3, 3}]9444
{1, 1, 1, 1, 3, 4}]9444
{1, 1, 1, 1, 3, 5}]180
{1, 1, 1, 1, 3, 6}]-24
{1, 1, 1, 1, 4, 1}]3
{1, 1, 1, 1, 4, 2}]-22
{1, 1, 1, 1, 4, 3}]59
{1, 1, 1, 1, 4, 4}]1024
{1, 1, 1, 1, 4, 5}]59
{1, 1, 1, 1, 4, 6}]-22
{1, 1, 1, 1, 4, 7}]3
{1, 1, 1, 2, 2, 2}]10792
{1, 1, 1, 2, 2, 3}]95648
{1, 1, 1, 2, 2, 4}]95648
{1, 1, 1, 2, 2, 5}]10792
{1, 1, 1, 2, 3, 2}]276
{1, 1, 1, 2, 3, 3}]43326
{1, 1, 1, 2, 3, 4}]125676
{1, 1, 1, 2, 3, 5}]43326
{1, 1, 1, 2, 3, 6}]276
{1, 1, 1, 2, 4, 2}]-48
{1, 1, 1, 2, 4, 3}]432
{1, 1, 1, 2, 4, 4}]22320
{1, 1, 1, 2, 4, 5}]22320
{1, 1, 1, 2, 4, 6}]432
{1, 1, 1, 2, 5, 2}]3
{1, 1, 1, 2, 5, 3}]-22
{1, 1, 1, 2, 5, 4}]59
{1, 1, 1, 2, 5, 5}]1024
{1, 1, 1, 3, 3, 3}]22680
{1, 1, 1, 3, 3, 4}]194664
{1, 1, 1, 3, 3, 5}]194664
{1, 1, 1, 3, 3, 6}]22680
{1, 1, 1, 3, 4, 3}]276
{1, 1, 1, 3, 4, 4}]43326
{1, 1, 1, 3, 4, 5}]125676
{1, 1, 1, 3, 5, 3}]-24
{1, 1, 1, 3, 5, 4}]180
{1, 1, 1, 4, 4, 4}]10792
{1, 1, 2, 2, 2, 2}]15902
{1, 1, 2, 2, 2, 3}]369646
{1, 1, 2, 2, 2, 4}]920760
{1, 1, 2, 2, 2, 5}]369646
{1, 1, 2, 2, 2, 6}]15902
{1, 1, 2, 2, 3, 2}]596
{1, 1, 2, 2, 3, 3}]210748
{1, 1, 2, 2, 3, 4}]1399712
{1, 1, 2, 2, 3, 5}]1399712
{1, 1, 2, 2, 3, 6}]210748
{1, 1, 2, 2, 4, 2}]-176
{1, 1, 2, 2, 4, 3}]3558
{1, 1, 2, 2, 4, 4}]360222
{1, 1, 2, 2, 4, 5}]964648
{1, 1, 2, 2, 5, 2}]36
{1, 1, 2, 2, 5, 3}]-400
{1, 1, 2, 2, 5, 4}]2560
{1, 1, 2, 2, 6, 2}]-4
{1, 1, 2, 2, 6, 3}]30
{1, 1, 2, 3, 3, 2}]2
{1, 1, 2, 3, 3, 3}]139918
{1, 1, 2, 3, 3, 4}]2449206
{1, 1, 2, 3, 3, 5}]5705460
{1, 1, 2, 3, 4, 3}]2676
{1, 1, 2, 3, 4, 4}]766084
{1, 1, 2, 3, 5, 3}]-376
{1, 1, 2, 4, 4, 3}]20
{1, 1, 3, 3, 3, 3}]112196
{1, 1, 3, 3, 3, 4}]4878540
{1, 1, 3, 3, 4, 3}]2775
{1, 2, 2, 2, 2, 2}]27600
{1, 2, 2, 2, 2, 3}]1585020
{1, 2, 2, 2, 2, 4}]8537376
{1, 2, 2, 2, 2, 5}]8537376
{1, 2, 2, 2, 2, 6}]1585020
{1, 2, 2, 2, 3, 2}]1344
{1, 2, 2, 2, 3, 3}]1097052
{1, 2, 2, 2, 3, 4}]14667648
{1, 2, 2, 2, 3, 5}]32044488
{1, 2, 2, 2, 4, 2}]-552
{1, 2, 2, 2, 4, 3}]26364
{1, 2, 2, 2, 4, 4}]4907940
{1, 2, 2, 2, 5, 2}]198
{1, 2, 2, 2, 5, 3}]-3960
{1, 2, 2, 2, 6, 2}]-48
{1, 2, 2, 3, 3, 2}]24
{1, 2, 2, 3, 3, 3}]878696
{1, 2, 2, 3, 3, 4}]28577520
{1, 2, 2, 3, 4, 2}]-2
{1, 2, 2, 3, 4, 3}]24120
{1, 2, 3, 3, 3, 3}]823008
{2, 2, 2, 2, 2, 2}]52740
{2, 2, 2, 2, 2, 3}]7545520
{2, 2, 2, 2, 2, 4}]80109420
{2, 2, 2, 2, 2, 5}]166265920
{2, 2, 2, 2, 3, 2}]2928
{2, 2, 2, 2, 3, 3}]6157524
{2, 2, 2, 2, 3, 4}]154063572
{2, 2, 2, 2, 4, 2}]-1338
{2, 2, 2, 2, 4, 3}]178908
{2, 2, 2, 2, 5, 2}]660
{2, 2, 2, 3, 3, 2}]142
{2, 2, 2, 3, 3, 3}]5734779
{2, 2, 2, 3, 4, 2}]-24

==> FirstGenus0Tables.tex <==
why no work
\begin{table}[p]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{4},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{4},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{4},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/6/.style={select equal part entry of={3}{4},column type = {|l},column name=\hfil $\bm p$},
display columns/7/.style={select equal part entry of={3}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{0, 0, 0, 0, 0, 1}]10
{0, 0, 0, 0, 1, 0}]12
{0, 0, 0, 0, 1, 1}]12
{0, 0, 0, 1, 1, 0}]1
{0, 0, 0, 1, 1, 1}]22
{0, 0, 0, 1, 1, 2}]1
{0, 0, 1, 1, 1, 1}]56
{0, 0, 1, 1, 1, 2}]56
{0, 0, 1, 1, 2, 1}]1
{0, 0, 1, 1, 2, 2}]22
{0, 0, 1, 1, 2, 3}]1
{0, 0, 1, 2, 2, 2}]12
{0, 0, 1, 2, 2, 3}]12
{0, 0, 2, 2, 2, 2}]10
{0, 0, 2, 2, 2, 3}]60
{0, 0, 2, 2, 2, 4}]10
{0, 0, 2, 2, 3, 3}]12
{0, 0, 2, 2, 3, 4}]12
{0, 0, 2, 3, 3, 3}]1
{0, 0, 2, 3, 3, 4}]22
{0, 0, 2, 3, 3, 5}]1
{0, 0, 3, 3, 3, 4}]56
{0, 0, 3, 3, 3, 5}]56
{0, 0, 3, 3, 4, 4}]1
{0, 0, 3, 3, 4, 5}]22
{0, 1, 1, 1, 1, 1}]174
{0, 1, 1, 1, 1, 2}]756
{0, 1, 1, 1, 1, 3}]174
{0, 1, 1, 1, 2, 1}]12
{0, 1, 1, 1, 2, 2}]540
{0, 1, 1, 1, 2, 3}]540
{0, 1, 1, 1, 2, 4}]12
{0, 1, 1, 1, 3, 1}]-2
{0, 1, 1, 1, 3, 2}]10
{0, 1, 1, 1, 3, 3}]96
{0, 1, 1, 1, 3, 4}]10
{0, 1, 1, 1, 3, 5}]-2
{0, 1, 1, 2, 2, 2}]474
{0, 1, 1, 2, 2, 3}]1852
{0, 1, 1, 2, 2, 4}]474
{0, 1, 1, 2, 3, 2}]12
{0, 1, 1, 2, 3, 3}]540
{0, 1, 1, 2, 3, 4}]540
{0, 1, 1, 2, 3, 5}]12
{0, 1, 1, 2, 4, 3}]1
{0, 1, 1, 2, 4, 4}]22
{0, 1, 1, 2, 4, 5}]1
{0, 1, 1, 3, 3, 3}]174
{0, 1, 1, 3, 3, 4}]756
{0, 1, 1, 3, 3, 5}]174
{0, 1, 1, 3, 4, 4}]56
{0, 1, 1, 3, 4, 5}]56
{0, 1, 1, 4, 4, 4}]1
{0, 1, 1, 4, 4, 5}]22
{0, 1, 2, 2, 2, 2}]540
{0, 1, 2, 2, 2, 3}]6708
{0, 1, 2, 2, 2, 4}]6708
{0, 1, 2, 2, 2, 5}]540
{0, 1, 2, 2, 3, 2}]22
{0, 1, 2, 2, 3, 3}]2796
{0, 1, 2, 2, 3, 4}]8860
{0, 1, 2, 2, 3, 5}]2796
{0, 1, 2, 2, 3, 6}]22
{0, 1, 2, 2, 4, 3}]56
{0, 1, 2, 2, 4, 4}]1344
{0, 1, 2, 2, 4, 5}]1344
{0, 1, 2, 2, 4, 6}]56
{0, 1, 2, 2, 5, 4}]1
{0, 1, 2, 2, 5, 5}]22
{0, 1, 2, 3, 3, 3}]1344
{0, 1, 2, 3, 3, 4}]13968
{0, 1, 2, 3, 3, 5}]13968
{0, 1, 2, 3, 3, 6}]1344
{0, 1, 2, 3, 4, 3}]22
{0, 1, 2, 3, 4, 4}]2796
{0, 1, 2, 3, 4, 5}]8860
{0, 1, 2, 3, 5, 4}]12
{0, 1, 2, 4, 4, 4}]540
{0, 1, 3, 3, 3, 3}]798
{0, 1, 3, 3, 3, 4}]25662
{0, 1, 3, 3, 3, 5}]69528
{0, 1, 3, 3, 4, 3}]12
{0, 1, 3, 3, 4, 4}]6708
{0, 2, 2, 2, 2, 2}]756
{0, 2, 2, 2, 2, 3}]25662
{0, 2, 2, 2, 2, 4}]69516
{0, 2, 2, 2, 2, 5}]25662
{0, 2, 2, 2, 2, 6}]756
{0, 2, 2, 2, 3, 2}]56
{0, 2, 2, 2, 3, 3}]13968
{0, 2, 2, 2, 3, 4}]103000
{0, 2, 2, 2, 3, 5}]103000
{0, 2, 2, 2, 3, 6}]13968
{0, 2, 2, 2, 4, 3}]756
{0, 2, 2, 2, 4, 4}]25662
{0, 2, 2, 2, 4, 5}]69516
{0, 2, 2, 2, 5, 4}]540
{0, 2, 2, 3, 3, 2}]1
{0, 2, 2, 3, 3, 3}]8860
{0, 2, 2, 3, 3, 4}]176251
{0, 2, 2, 3, 3, 5}]425712
{0, 2, 2, 3, 4, 3}]540
{0, 2, 2, 3, 4, 4}]54504
{0, 2, 2, 4, 4, 3}]10
{0, 2, 3, 3, 3, 3}]6708
{0, 2, 3, 3, 3, 4}]342924
{0, 2, 3, 3, 4, 3}]474
{0, 3, 3, 3, 3, 3}]6204
{1, 1, 1, 1, 1, 1}]700
{1, 1, 1, 1, 1, 2}]8900
{1, 1, 1, 1, 1, 3}]8900
{1, 1, 1, 1, 1, 4}]700
{1, 1, 1, 1, 2, 1}]66
{1, 1, 1, 1, 2, 2}]8892
{1, 1, 1, 1, 2, 3}]27492
{1, 1, 1, 1, 2, 4}]8892
{1, 1, 1, 1, 2, 5}]66
{1, 1, 1, 1, 3, 1}]-24
{1, 1, 1, 1, 3, 2}]180
{1, 1, 1, 1, 3, 3}]9444
{1, 1, 1, 1, 3, 4}]9444
{1, 1, 1, 1, 3, 5}]180
{1, 1, 1, 1, 3, 6}]-24
{1, 1, 1, 1, 4, 1}]3
{1, 1, 1, 1, 4, 2}]-22
{1, 1, 1, 1, 4, 3}]59
{1, 1, 1, 1, 4, 4}]1024
{1, 1, 1, 1, 4, 5}]59
{1, 1, 1, 1, 4, 6}]-22
{1, 1, 1, 1, 4, 7}]3
{1, 1, 1, 2, 2, 2}]10792
{1, 1, 1, 2, 2, 3}]95648
{1, 1, 1, 2, 2, 4}]95648
{1, 1, 1, 2, 2, 5}]10792
{1, 1, 1, 2, 3, 2}]276
{1, 1, 1, 2, 3, 3}]43326
{1, 1, 1, 2, 3, 4}]125676
{1, 1, 1, 2, 3, 5}]43326
{1, 1, 1, 2, 3, 6}]276
{1, 1, 1, 2, 4, 2}]-48
{1, 1, 1, 2, 4, 3}]432
{1, 1, 1, 2, 4, 4}]22320
{1, 1, 1, 2, 4, 5}]22320
{1, 1, 1, 2, 4, 6}]432
{1, 1, 1, 2, 5, 2}]3
{1, 1, 1, 2, 5, 3}]-22
{1, 1, 1, 2, 5, 4}]59
{1, 1, 1, 2, 5, 5}]1024
{1, 1, 1, 3, 3, 3}]22680
{1, 1, 1, 3, 3, 4}]194664
{1, 1, 1, 3, 3, 5}]194664
{1, 1, 1, 3, 3, 6}]22680
{1, 1, 1, 3, 4, 3}]276
{1, 1, 1, 3, 4, 4}]43326
{1, 1, 1, 3, 4, 5}]125676
{1, 1, 1, 3, 5, 3}]-24
{1, 1, 1, 3, 5, 4}]180
{1, 1, 1, 4, 4, 4}]10792
{1, 1, 2, 2, 2, 2}]15902
{1, 1, 2, 2, 2, 3}]369646
{1, 1, 2, 2, 2, 4}]920760
{1, 1, 2, 2, 2, 5}]369646
{1, 1, 2, 2, 2, 6}]15902
{1, 1, 2, 2, 3, 2}]596
{1, 1, 2, 2, 3, 3}]210748
{1, 1, 2, 2, 3, 4}]1399712
{1, 1, 2, 2, 3, 5}]1399712
{1, 1, 2, 2, 3, 6}]210748
{1, 1, 2, 2, 4, 2}]-176
{1, 1, 2, 2, 4, 3}]3558
{1, 1, 2, 2, 4, 4}]360222
{1, 1, 2, 2, 4, 5}]964648
{1, 1, 2, 2, 5, 2}]36
{1, 1, 2, 2, 5, 3}]-400
{1, 1, 2, 2, 5, 4}]2560
{1, 1, 2, 2, 6, 2}]-4
{1, 1, 2, 2, 6, 3}]30
{1, 1, 2, 3, 3, 2}]2
{1, 1, 2, 3, 3, 3}]139918
{1, 1, 2, 3, 3, 4}]2449206
{1, 1, 2, 3, 3, 5}]5705460
{1, 1, 2, 3, 4, 3}]2676
{1, 1, 2, 3, 4, 4}]766084
{1, 1, 2, 3, 5, 3}]-376
{1, 1, 2, 4, 4, 3}]20
{1, 1, 3, 3, 3, 3}]112196
{1, 1, 3, 3, 3, 4}]4878540
{1, 1, 3, 3, 4, 3}]2775
{1, 2, 2, 2, 2, 2}]27600
{1, 2, 2, 2, 2, 3}]1585020
{1, 2, 2, 2, 2, 4}]8537376
{1, 2, 2, 2, 2, 5}]8537376
{1, 2, 2, 2, 2, 6}]1585020
{1, 2, 2, 2, 3, 2}]1344
{1, 2, 2, 2, 3, 3}]1097052
{1, 2, 2, 2, 3, 4}]14667648
{1, 2, 2, 2, 3, 5}]32044488
{1, 2, 2, 2, 4, 2}]-552
{1, 2, 2, 2, 4, 3}]26364
{1, 2, 2, 2, 4, 4}]4907940
{1, 2, 2, 2, 5, 2}]198
{1, 2, 2, 2, 5, 3}]-3960
{1, 2, 2, 2, 6, 2}]-48
{1, 2, 2, 3, 3, 2}]24
{1, 2, 2, 3, 3, 3}]878696
{1, 2, 2, 3, 3, 4}]28577520
{1, 2, 2, 3, 4, 2}]-2
{1, 2, 2, 3, 4, 3}]24120
{1, 2, 3, 3, 3, 3}]823008
{2, 2, 2, 2, 2, 2}]52740
{2, 2, 2, 2, 2, 3}]7545520
{2, 2, 2, 2, 2, 4}]80109420
{2, 2, 2, 2, 2, 5}]166265920
{2, 2, 2, 2, 3, 2}]2928
{2, 2, 2, 2, 3, 3}]6157524
{2, 2, 2, 2, 3, 4}]154063572
{2, 2, 2, 2, 4, 2}]-1338
{2, 2, 2, 2, 4, 3}]178908
{2, 2, 2, 2, 5, 2}]660
{2, 2, 2, 3, 3, 2}]142
{2, 2, 2, 3, 3, 3}]5734779
{2, 2, 2, 3, 4, 2}]-24
}
}
\end{adjustbox}
\vskip10pt
\capt{5in}{tab:Instanton_Numbers_6_36}{The genus~0 instanton numbers of total degree $\leqslant 15$ for the family \eqref{eq:CICY_6_36}. The numbers not in this list are either zero, or given by those in the table after a permutation of the first five indices. The sixth index \textbf{cannot} be exchanged with the others.}
\end{table}
\begin{table}[p]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{3},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{0, 0, 0, 0, 0, 0, 1}]10
{0, 0, 0, 0, 1, 0, 0}]6
{0, 0, 0, 0, 1, 0, 1}]6
{0, 0, 0, 0, 1, 1, 1}]6
{0, 0, 0, 1, 1, 0, 1}]1
{0, 0, 0, 1, 1, 1, 1}]20
{0, 0, 0, 1, 1, 1, 2}]1
{0, 0, 1, 1, 1, 1, 1}]28
{0, 0, 1, 1, 1, 1, 2}]28
{0, 0, 1, 1, 1, 2, 2}]28
{0, 0, 1, 1, 2, 1, 2}]1
{0, 0, 1, 1, 2, 2, 2}]20
{0, 0, 1, 1, 2, 2, 3}]1
{0, 0, 1, 2, 2, 2, 2}]6
{0, 0, 1, 2, 2, 2, 3}]6
{0, 0, 1, 2, 2, 3, 3}]6
{0, 0, 2, 2, 2, 2, 3}]10
{0, 0, 2, 2, 2, 3, 3}]40
{0, 0, 2, 2, 2, 3, 4}]10
{0, 0, 2, 2, 3, 3, 3}]6
{0, 1, 1, 1, 1, 1, 1}]24
{0, 1, 1, 1, 1, 1, 2}]126
{0, 1, 1, 1, 1, 1, 3}]24
{0, 1, 1, 1, 1, 2, 2}]504
{0, 1, 1, 1, 1, 2, 3}]126
{0, 1, 1, 1, 1, 3, 3}]24
{0, 1, 1, 1, 2, 1, 2}]6
{0, 1, 1, 1, 2, 1, 3}]6
{0, 1, 1, 1, 2, 2, 2}]264
{0, 1, 1, 1, 2, 2, 3}]264
{0, 1, 1, 1, 2, 2, 4}]6
{0, 1, 1, 1, 2, 3, 3}]264
{0, 1, 1, 1, 2, 3, 4}]6
{0, 1, 1, 1, 3, 1, 3}]-2
{0, 1, 1, 1, 3, 2, 3}]10
{0, 1, 1, 1, 3, 3, 3}]80
{0, 1, 1, 1, 3, 3, 4}]10
{0, 1, 1, 2, 2, 2, 2}]72
{0, 1, 1, 2, 2, 2, 3}]330
{0, 1, 1, 2, 2, 2, 4}]72
{0, 1, 1, 2, 2, 3, 3}]1192
{0, 1, 1, 2, 2, 3, 4}]330
{0, 1, 1, 2, 3, 2, 3}]6
{0, 1, 1, 2, 3, 2, 4}]6
{0, 1, 1, 2, 3, 3, 3}]264
{0, 1, 2, 2, 2, 2, 2}]6
{0, 1, 2, 2, 2, 2, 3}]264
{0, 1, 2, 2, 2, 2, 4}]264
{0, 1, 2, 2, 2, 3, 3}]3090
{0, 1, 2, 2, 3, 2, 3}]1
{0, 2, 2, 2, 2, 2, 3}]126
{1, 1, 1, 1, 1, 1, 1}]20
{1, 1, 1, 1, 1, 1, 2}]330
{1, 1, 1, 1, 1, 1, 3}]330
{1, 1, 1, 1, 1, 1, 4}]20
{1, 1, 1, 1, 1, 2, 2}]4120
{1, 1, 1, 1, 1, 2, 3}]4120
{1, 1, 1, 1, 1, 2, 4}]330
{1, 1, 1, 1, 1, 3, 3}]4120
{1, 1, 1, 1, 1, 3, 4}]330
{1, 1, 1, 1, 1, 4, 4}]20
{1, 1, 1, 1, 2, 1, 2}]15
{1, 1, 1, 1, 2, 1, 3}]36
{1, 1, 1, 1, 2, 1, 4}]15
{1, 1, 1, 1, 2, 2, 2}]1692
{1, 1, 1, 1, 2, 2, 3}]5478
{1, 1, 1, 1, 2, 2, 4}]1692
{1, 1, 1, 1, 2, 2, 5}]15
{1, 1, 1, 1, 2, 3, 3}]16464
{1, 1, 1, 1, 2, 3, 4}]5478
{1, 1, 1, 1, 3, 1, 3}]-12
{1, 1, 1, 1, 3, 1, 4}]-12
{1, 1, 1, 1, 3, 2, 3}]90
{1, 1, 1, 1, 3, 2, 4}]90
{1, 1, 1, 1, 3, 3, 3}]4644
{1, 1, 1, 1, 4, 1, 4}]3
{1, 1, 1, 2, 2, 2, 2}]480
{1, 1, 1, 2, 2, 2, 3}]4916
{1, 1, 1, 2, 2, 2, 4}]4916
{1, 1, 1, 2, 2, 3, 3}]42908
{1, 1, 1, 2, 3, 2, 3}]54
{1, 1, 2, 2, 2, 2, 2}]80
{1, 1, 2, 2, 2, 2, 3}]3293
{1, 2, 2, 2, 2, 2, 2}]6
}
}
\end{adjustbox}
\vskip10pt
\capt{5in}{tab:Instanton_Numbers_7_27}{The genus~0 instanton numbers of total degree $\leqslant 13$ for the family \eqref{eq:CICY_7_27}. The numbers not in this list are either zero, or given by those in the table after a permutations of the first five and last two indices. The sixth and seventh indices \textbf{cannot} be exchanged with the first five.}
\end{table}
\begin{table}[p]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{3},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{1, 0, 0, 0}]48
{1, 1, 0, 0}]160
{1, 1, 1, 0}]2432
{1, 1, 1, 1}]86016
{2, 1, 0, 0}]48
{2, 1, 1, 0}]5056
{2, 1, 1, 1}]518784
{2, 2, 0, 0}]128
{2, 2, 1, 0}]34640
{2, 2, 1, 1}]7037184
{2, 2, 2, 0}]507904
{2, 2, 2, 1}]171165840
{2, 2, 2, 2}]6547900416
{3, 1, 1, 0}]2432
{3, 1, 1, 1}]899072
{3, 2, 0, 0}]48
{3, 2, 1, 0}]61824
{3, 2, 1, 1}]28639616
{3, 2, 2, 0}]2089008
{3, 2, 2, 1}]1297013760
{3, 2, 2, 2}]80605022416
{3, 3, 0, 0}]160
{3, 3, 1, 0}]308352
{3, 3, 1, 1}]241754112
{3, 3, 2, 0}]17677056
{3, 3, 2, 1}]17200647552
{3, 3, 2, 2}]1557963029504
{3, 3, 3, 0}]252810752
{3, 3, 3, 1}]352652451840
{3, 3, 3, 2}]43431181213824
{3, 3, 3, 3}]1646607181615104
{4, 1, 1, 0}]160
{4, 1, 1, 1}]518784
{4, 2, 1, 0}]34640
{4, 2, 1, 1}]44662400
{4, 2, 2, 0}]3265280
{4, 2, 2, 1}]4042603552
{4, 2, 2, 2}]426305384448
{4, 3, 0, 0}]48
{4, 3, 1, 0}]508160
{4, 3, 1, 1}]789382400
{4, 3, 2, 0}]57521568
{4, 3, 2, 1}]94371041920
{4, 3, 2, 2}]13002686858864
{4, 3, 3, 0}]1424625024
{4, 3, 3, 1}]3031512413312
{4, 3, 3, 2}]527889850255360
{4, 3, 3, 3}]27526058324060160
{4, 4, 0, 0}]128
{4, 4, 1, 0}]2089008
{4, 4, 1, 1}]4985888864
{4, 4, 2, 0}]360824832
{4, 4, 2, 1}]871452197440
{4, 4, 2, 2}]166647022068736
{4, 4, 3, 0}]13391051328
{4, 4, 3, 1}]39844405855232
{4, 4, 3, 2}]9199812356321968
{4, 4, 3, 3}]627205272329861504
{4, 4, 4, 0}]188051928064
{4, 4, 4, 1}]741058165634496
{4, 4, 4, 2}]217057048330727424
{4, 4, 4, 3}]18647281489625577504
{4, 4, 4, 4}]699794636853614635008
{5, 1, 1, 1}]86016
{5, 2, 1, 0}]5056
{5, 2, 1, 1}]28639616
{5, 2, 2, 0}]2089008
{5, 2, 2, 1}]5834714624
{5, 2, 2, 2}]1108729141920
{5, 3, 1, 0}]308352
{5, 3, 1, 1}]1154723840
{5, 3, 2, 0}]84056832
{5, 3, 2, 1}]249714336000
{5, 3, 2, 2}]54663940002816
{5, 3, 3, 0}]3808483584
{5, 3, 3, 1}]12944311033856
{5, 3, 3, 2}]3295227059205504
{5, 3, 3, 3}]240139807447941120
{5, 4, 0, 0}]48
{5, 4, 1, 0}]3265984
{5, 4, 1, 1}]14129065088
{5, 4, 2, 0}]1017784976
{5, 4, 2, 1}]3874428076928
{5, 4, 2, 2}]1074177329475184
{5, 4, 3, 0}]59821118208
{5, 4, 3, 1}]260287936814720
{5, 4, 3, 2}]82385600163793920
{5, 4, 3, 3}]7471070109015318656
{5, 4, 4, 0}]1268723299376
{5, 4, 4, 1}]6894039650704512
{5, 4, 4, 2}]2643331064630855200
{5, 4, 4, 3}]291051848701788699648
{5, 4, 4, 4}]13862614815470765167056
{5, 5, 0, 0}]160
{5, 5, 1, 0}]11746432
{5, 5, 1, 1}]73320878080
{5, 5, 2, 0}]5243776704
{5, 5, 2, 1}]27965750549248
{5, 5, 2, 2}]10380731579151872
{5, 5, 3, 0}]432161466624
{5, 5, 3, 1}]2545321829650432
{5, 5, 3, 2}]1042877238127097984
{5, 5, 3, 3}]120304302520611954688
{5, 5, 4, 0}]12709250594240
{5, 5, 4, 1}]90222224188616064
{5, 5, 4, 2}]43400958203031979648
{5, 5, 4, 3}]5917889244182186813696
{5, 5, 4, 4}]347399539693965379619648
{5, 5, 5, 0}]176223512332928
{5, 5, 5, 1}]1575672398623395840
{5, 5, 5, 2}]922075476759511908864
{5, 5, 5, 3}]151692725887218685190144
{5, 5, 5, 4}]10726096697730587601447552
{5, 5, 5, 5}]399456970261757309912334336
{6, 1, 1, 1}]2432
{6, 2, 1, 0}]48
{6, 2, 1, 1}]7037184
{6, 2, 2, 0}]507904
{6, 2, 2, 1}]4042603552
{6, 2, 2, 2}]1514352078848
{6, 3, 1, 0}]61824
{6, 3, 1, 1}]789382400
{6, 3, 2, 0}]57521568
{6, 3, 2, 1}]342823329792
{6, 3, 2, 2}]125771915722896
{6, 3, 3, 0}]5243776704
{6, 3, 3, 1}]30008993843584
{6, 3, 3, 2}]11575415612576768
{6, 3, 3, 3}]1203234568961692800
{6, 4, 1, 0}]2089008
{6, 4, 1, 1}]19804670208
{6, 4, 2, 0}]1424616960
{6, 4, 2, 1}]9173232641616
{6, 4, 2, 2}]3846287763468288
{6, 4, 3, 0}]141793830384
{6, 4, 3, 1}]938779827042688
{6, 4, 3, 2}]419700792333851408
{6, 4, 3, 3}]51546803704385918976
{6, 4, 4, 0}]4650991239168
{6, 4, 4, 1}]35938232545114592
{6, 4, 4, 2}]18502170216819978240
{6, 4, 4, 3}]2653048822718080612368
{6, 4, 4, 4}]161629518930438998396928
{6, 5, 0, 0}]48
{6, 5, 1, 0}]17677056
{6, 5, 1, 1}]188011416064
{6, 5, 2, 0}]13391051328
{6, 5, 2, 1}]107087122937856
{6, 5, 2, 2}]55530466229981712
{6, 5, 3, 0}]1651763971584
{6, 5, 3, 1}]13704006681994624
{6, 5, 3, 2}]7493044028521115648
{6, 5, 3, 3}]1120675249090550046720
{6, 5, 4, 0}]69188204803344
{6, 5, 4, 1}]661446106005076224
{6, 5, 4, 2}]409473371380697240000
{6, 5, 4, 3}]70283944963932592401152
{6, 5, 4, 4}]5129348718881933358532960
{6, 5, 5, 0}]1335543626995200
{6, 5, 5, 1}]15470217373819587584
{6, 5, 5, 2}]11284911987863253245440
{6, 5, 5, 3}]2276112606495732006202112
{6, 5, 5, 4}]195588673772290431107673344
{6, 6, 0, 0}]128
{6, 6, 1, 0}]57521568
{6, 6, 1, 1}]845112783616
{6, 6, 2, 0}]59821080576
{6, 6, 2, 1}]645375311627376
{6, 6, 2, 2}]435566317842866176
{6, 6, 3, 0}]9911375239392
{6, 6, 3, 1}]108118212077621248
{6, 6, 3, 2}]74937314945510009952
{6, 6, 3, 3}]13961655375523769282816
{6, 6, 4, 0}]549828820220928
{6, 6, 4, 1}]6736033668350881952
{6, 6, 4, 2}]5160552306598346379264
{6, 6, 4, 3}]1080443741007758375555472
{6, 6, 4, 4}]95469681182710628821921792
{6, 6, 5, 0}]13962620228584512
{6, 6, 5, 1}]201987366061445211648
{6, 6, 5, 2}]178213464042928851755872
{6, 6, 5, 3}]42979893686208656793686016
{6, 6, 6, 0}]191827050005069824
{6, 6, 6, 1}]3375664486259351631456
{6, 6, 6, 2}]3521325683147770386726912
{7, 2, 1, 1}]518784
{7, 2, 2, 0}]34640
{7, 2, 2, 1}]1297013760
{7, 2, 2, 2}]1108729141920
{7, 3, 1, 0}]2432
{7, 3, 1, 1}]241754112
{7, 3, 2, 0}]17677056
{7, 3, 2, 1}]249714336000
{7, 3, 2, 2}]165296580806656
{7, 3, 3, 0}]3808483584
{7, 3, 3, 1}]39529406119936
{7, 3, 3, 2}]24136954745543808
{7, 3, 3, 3}]3672469607846903808
{7, 4, 1, 0}]508160
{7, 4, 1, 1}]14129065088
{7, 4, 2, 0}]1017784976
{7, 4, 2, 1}]12163074768640
{7, 4, 2, 2}]8102781267426048
{7, 4, 3, 0}]188051992832
{7, 4, 3, 1}]1984799528343552
{7, 4, 3, 2}]1294128535920058368
{7, 4, 3, 3}]219681085367035373952
{7, 4, 4, 0}]9911375239392
{7, 4, 4, 1}]112338620588205056
{7, 4, 4, 2}]79594696896349282688
{7, 4, 4, 3}]15110868372965862621696
{7, 4, 4, 4}]1189045428745766422260768
{7, 5, 1, 0}]11746432
{7, 5, 1, 1}]255547666432
{7, 5, 2, 0}]18178255616
{7, 5, 2, 1}]233839970568832
{7, 5, 2, 2}]176514847485662208
{7, 5, 3, 0}]3600925105536
{7, 5, 3, 1}]43715576259518464
{7, 5, 3, 2}]32805238780261668736
{7, 5, 3, 3}]6480417642541472432128
{7, 5, 4, 0}]221844802863872
{7, 5, 4, 1}]2932079676057142912
{7, 5, 4, 2}]2387966888748874810112
{7, 5, 4, 3}]523912487781610422477568
{7, 5, 4, 4}]47981652609161486365088768
{7, 5, 5, 0}]6036801603750144
{7, 5, 5, 1}]92621472022310780928
{7, 5, 5, 2}]85897234681261670146944
{7, 5, 5, 3}]21540883712581909578244096
{7, 6, 0, 0}]48
{7, 6, 1, 0}]84056832
{7, 6, 1, 1}]2010040031104
{7, 6, 2, 0}]141793830384
}
}
\end{adjustbox}
\vskip10pt
\capt{5in}{tab:Instanton_Numbers_4_68}{The genus~0 instanton numbers of total degree $\leqslant 20$ for the family \eqref{eq:CICY_4_68}. The numbers not in this list are either zero, or given by those in the table after a permutation indices.}
\end{table}
\begin{table}[p]\notag
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{3},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{7, 6, 2, 1}]2208595900084224
{7, 6, 2, 2}]2021884379122016048
{7, 6, 3, 0}]33789217322496
{7, 6, 3, 1}]503495581721955456
{7, 6, 3, 2}]455218569908331757568
{7, 6, 3, 3}]107719074363142059583360
{7, 6, 4, 0}]2566483940906640
{7, 6, 4, 1}]41379145350412949504
{7, 6, 4, 2}]40123559676936131346720
{7, 6, 4, 3}]10410193126310745548984320
{7, 6, 5, 0}]87046894784712960
{7, 6, 5, 1}]1607540052866407577728
{7, 6, 5, 2}]1749693070862210564431872
{7, 6, 6, 0}]1576912001012723760
{7, 6, 6, 1}]34462954830661856456704
{7, 7, 0, 0}]160
{7, 7, 1, 0}]252810752
{7, 7, 1, 1}]8087692763136
{7, 7, 2, 0}]567589415680
{7, 7, 2, 1}]11584959011321216
{7, 7, 2, 2}]13491384176760961024
{7, 7, 3, 0}]176223512332928
{7, 7, 3, 1}]3369477175185817600
{7, 7, 3, 2}]3792683314958877584384
{7, 7, 3, 3}]1099277650161884440166400
{7, 7, 4, 0}]17175761255142144
{7, 7, 4, 1}]348295401563531685632
{7, 7, 4, 2}]412395106599944043177984
{7, 7, 5, 0}]740932627227834624
{7, 7, 5, 1}]16875996286670980751360
{7, 7, 6, 0}]16999688846773790208
{8, 2, 1, 1}]5056
{8, 2, 2, 0}]128
{8, 2, 2, 1}]171165840
{8, 2, 2, 2}]426305384448
{8, 3, 1, 1}]28639616
{8, 3, 2, 0}]2089008
{8, 3, 2, 1}]94371041920
{8, 3, 2, 2}]125771915722896
{8, 3, 3, 0}]1424625024
{8, 3, 3, 1}]30008993843584
{8, 3, 3, 2}]30743146145765888
{8, 3, 3, 3}]7079306295276204288
{8, 4, 1, 0}]34640
{8, 4, 1, 1}]4985888864
{8, 4, 2, 0}]360824832
{8, 4, 2, 1}]9173232641616
{8, 4, 2, 2}]10353839703716352
{8, 4, 3, 0}]141793830384
{8, 4, 3, 1}]2538964516666880
{8, 4, 3, 2}]2508525839463392816
{8, 4, 3, 3}]602927912105481193728
{8, 4, 4, 0}]12709250181888
{8, 4, 4, 1}]219342311907269104
{8, 4, 4, 2}]219737543096535650304
{8, 4, 4, 3}]56255611905947864806512
{8, 4, 4, 4}]5785403639953201842686976
{8, 5, 1, 0}]3265984
{8, 5, 1, 1}]188011416064
{8, 5, 2, 0}]13391051328
{8, 5, 2, 1}]302207140853120
{8, 5, 2, 2}]347926332689829040
{8, 5, 3, 0}]4650991497216
{8, 5, 3, 1}]86320414207198848
{8, 5, 3, 2}]91592941667768938752
{8, 5, 3, 3}]24378159414883707592448
{8, 5, 4, 0}]439063136203008
{8, 5, 4, 1}]8247835975441925056
{8, 5, 4, 2}]9033581369124138593840
{8, 5, 4, 3}]2573204027887680476759296
{8, 5, 5, 0}]17175761255142144
{8, 5, 5, 1}]356496506323192211328
{8, 5, 5, 2}]428090722447387987896384
{8, 6, 1, 0}]57521568
{8, 6, 1, 1}]2668638725632
{8, 6, 2, 0}]188051928064
{8, 6, 2, 1}]4533354437642480
{8, 6, 2, 2}]5860852677002366976
{8, 6, 3, 0}]69188204803344
{8, 6, 3, 1}]1462074329960965376
{8, 6, 3, 2}]1771264367116721723008
{8, 6, 3, 3}]542307422558027394152960
{8, 6, 4, 0}]7456149925576704
{8, 6, 4, 1}]162132923614385349360
{8, 6, 4, 2}]203054957441346394726912
{8, 6, 5, 0}]343945562331791376
{8, 6, 5, 1}]8263402711793164324608
{8, 6, 6, 0}]8277365987776740864
{8, 7, 0, 0}]48
{8, 7, 1, 0}]360828928
{8, 7, 1, 1}]18129723322752
{8, 7, 2, 0}]1268723299376
{8, 7, 2, 1}]36298079877646592
{8, 7, 2, 2}]55987725237356145792
{8, 7, 3, 0}]549828822442752
{8, 7, 3, 1}]14005384303898305024
{8, 7, 3, 2}]20171041734451334944000
{8, 7, 4, 0}]71290241748070896
{8, 7, 4, 1}]1864208769268632504064
{8, 7, 5, 0}]3988612138839842816
{8, 8, 0, 0}]128
{8, 8, 1, 0}]1017784976
{8, 8, 1, 1}]66748924807328
{8, 8, 2, 0}]4650991239168
{8, 8, 2, 1}]170418886235419696
{8, 8, 2, 2}]328173467451404489600
{8, 8, 3, 0}]2566483940906640
{8, 8, 3, 1}]82211057906371385344
{8, 8, 4, 0}]417176124089319424
{9, 2, 2, 1}]7037184
{9, 2, 2, 2}]80605022416
{9, 3, 1, 1}]899072
{9, 3, 2, 0}]61824
{9, 3, 2, 1}]17200647552
{9, 3, 2, 2}]54663940002816
{9, 3, 3, 0}]252810752
{9, 3, 3, 1}]12944311033856
{9, 3, 3, 2}]24136954745543808
{9, 3, 3, 3}]8791828001566988288
{9, 4, 1, 0}]160
{9, 4, 1, 1}]789382400
{9, 4, 2, 0}]57521568
{9, 4, 2, 1}]3874428076928
{9, 4, 2, 2}]8102781267426048
{9, 4, 3, 0}]59821118208
{9, 4, 3, 1}]1984799528343552
{9, 4, 3, 2}]3120841582270747392
{9, 4, 3, 3}]1094190143621388343680
{9, 4, 4, 0}]9911375239392
{9, 4, 4, 1}]273504607073902144
{9, 4, 4, 2}]400065629964453039984
{9, 4, 4, 3}]141106319957374906048512
{9, 5, 1, 0}]308352
{9, 5, 1, 1}]73320878080
{9, 5, 2, 0}]5243776704
{9, 5, 2, 1}]233839970568832
{9, 5, 2, 2}]435172594319284224
{9, 5, 3, 0}]3600925105536
{9, 5, 3, 1}]108024514779267072
{9, 5, 3, 2}]167816512674800089472
{9, 5, 3, 3}]61564588462323994361856
{9, 5, 4, 0}]549828822442752
{9, 5, 4, 1}]15172240325024688384
{9, 5, 4, 2}]22894439058514947334656
{9, 5, 5, 0}]31786723861681536
{9, 5, 5, 1}]913426712060194627584
{9, 6, 1, 0}]17677056
{9, 6, 1, 1}]2010040031104
{9, 6, 2, 0}]141793830384
{9, 6, 2, 1}]5744002412760576
{9, 6, 2, 2}]10966073503132221968
{9, 6, 3, 0}]87594475420800
{9, 6, 3, 1}]2738079662657568640
{9, 6, 3, 2}]4572692498129982156800
{9, 6, 4, 0}]13962620228584512
{9, 6, 4, 1}]420332107728557286912
{9, 6, 5, 0}]895919580397273344
{9, 7, 1, 0}]252810752
{9, 7, 1, 1}]23624438407168
{9, 7, 2, 0}]1651763971584
{9, 7, 2, 1}]70930323016569984
{9, 7, 2, 2}]150750588373893541888
{9, 7, 3, 0}]1071736381056384
{9, 7, 3, 1}]37743466871928029184
{9, 7, 4, 0}]191827050036601856
{9, 8, 0, 0}]48
{9, 8, 1, 0}]1424625024
{9, 8, 1, 1}]142582803775232
{9, 8, 2, 0}]9911375239392
{9, 8, 2, 1}]497106580728095936
{9, 8, 3, 0}]7456149932740608
{9, 9, 0, 0}]160
{9, 9, 1, 0}]3808483584
{9, 9, 1, 1}]487860526727168
{9, 9, 2, 0}]33789217322496
{10, 2, 2, 1}]34640
{10, 2, 2, 2}]6547900416
{10, 3, 1, 1}]2432
{10, 3, 2, 0}]48
{10, 3, 2, 1}]1297013760
{10, 3, 2, 2}]13002686858864
{10, 3, 3, 0}]17677056
{10, 3, 3, 1}]3031512413312
{10, 3, 3, 2}]11575415612576768
{10, 3, 3, 3}]7079306295276204288
{10, 4, 1, 1}]44662400
{10, 4, 2, 0}]3265280
{10, 4, 2, 1}]871452197440
{10, 4, 2, 2}]3846287763468288
{10, 4, 3, 0}]13391051328
{10, 4, 3, 1}]938779827042688
{10, 4, 3, 2}]2508525839463392816
{10, 4, 3, 3}]1332539766738727936000
{10, 4, 4, 0}]4650991239168
{10, 4, 4, 1}]219342311907269104
{10, 4, 4, 2}]487713798985291233280
{10, 5, 1, 0}]5056
{10, 5, 1, 1}]14129065088
{10, 5, 2, 0}]1017784976
{10, 5, 2, 1}]107087122937856
{10, 5, 2, 2}]347926332689829040
{10, 5, 3, 0}]1651763971584
{10, 5, 3, 1}]86320414207198848
{10, 5, 3, 2}]204999947699695388672
{10, 5, 4, 0}]439063136203008
{10, 5, 4, 1}]18557339208009894656
{10, 5, 5, 0}]38952597058723520
{10, 6, 1, 0}]2089008
{10, 6, 1, 1}]845112783616
{10, 6, 2, 0}]59821080576
{10, 6, 2, 1}]4533354437642480
{10, 6, 2, 2}]13486794785676976128
{10, 6, 3, 0}]69188204803344
{10, 6, 3, 1}]3368380766765580288
{10, 6, 4, 0}]17175761244601344
{10, 7, 1, 0}]84056832
{10, 7, 1, 1}]18129723322752
{10, 7, 2, 0}]1268723299376
{10, 7, 2, 1}]88462669038163968
{10, 7, 3, 0}]1335543626995200
{10, 8, 1, 0}]1017784976
{10, 8, 1, 1}]182970871579264
{10, 8, 2, 0}]12709250181888
{10, 9, 0, 0}]48
{10, 9, 1, 0}]5243776704
{10, 10, 0, 0}]128
{11, 2, 2, 2}]171165840
{11, 3, 2, 1}]28639616
{11, 3, 2, 2}]1557963029504
{11, 3, 3, 0}]308352
{11, 3, 3, 1}]352652451840
{11, 3, 3, 2}]3295227059205504
{11, 3, 3, 3}]3672469607846903808
{11, 4, 1, 1}]518784
}
}
\end{adjustbox}
\vskip10pt
\caption*{\tref{tab:Instanton_Numbers_4_68} continued.}
\end{table}
\begin{table}[p]\notag
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{3},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{11, 4, 2, 0}]34640
{11, 4, 2, 1}]94371041920
{11, 4, 2, 2}]1074177329475184
{11, 4, 3, 0}]1424625024
{11, 4, 3, 1}]260287936814720
{11, 4, 3, 2}]1294128535920058368
{11, 4, 4, 0}]1268723299376
{11, 4, 4, 1}]112338620588205056
{11, 5, 1, 1}]1154723840
{11, 5, 2, 0}]84056832
{11, 5, 2, 1}]27965750549248
{11, 5, 2, 2}]176514847485662208
{11, 5, 3, 0}]432161466624
{11, 5, 3, 1}]43715576259518464
{11, 5, 4, 0}]221844802863872
{11, 6, 1, 0}]61824
{11, 6, 1, 1}]188011416064
{11, 6, 2, 0}]13391051328
{11, 6, 2, 1}]2208595900084224
{11, 6, 3, 0}]33789217322496
{11, 7, 1, 0}]11746432
{11, 7, 1, 1}]8087692763136
{11, 7, 2, 0}]567589415680
{11, 8, 1, 0}]360828928
{12, 2, 2, 2}]507904
{12, 3, 2, 1}]61824
{12, 3, 2, 2}]80605022416
{12, 3, 3, 0}]160
{12, 3, 3, 1}]17200647552
{12, 3, 3, 2}]527889850255360
{12, 4, 1, 1}]160
{12, 4, 2, 1}]4042603552
{12, 4, 2, 2}]166647022068736
{12, 4, 3, 0}]57521568
{12, 4, 3, 1}]39844405855232
{12, 4, 4, 0}]188051928064
{12, 5, 1, 1}]28639616
{12, 5, 2, 0}]2089008
{12, 5, 2, 1}]3874428076928
{12, 5, 3, 0}]59821118208
{12, 6, 1, 0}]48
{12, 6, 1, 1}]19804670208
{12, 6, 2, 0}]1424616960
{12, 7, 1, 0}]508160
{13, 3, 2, 2}]1297013760
{13, 3, 3, 1}]241754112
{13, 4, 2, 1}]44662400
{13, 4, 3, 0}]508160
{13, 5, 1, 1}]86016
{13, 5, 2, 0}]5056
}
}
\end{adjustbox}
\vskip10pt
\caption*{\tref{tab:Instanton_Numbers_4_68} continued.}
\end{table}
\begin{table}[p]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{3},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{0, 1}]50
{1, 1}]650
{1, 2}]1475
{2, 2}]29350
{1, 3}]650
{2, 3}]148525
{3, 3}]3270050
{1, 4}]50
{2, 4}]250550
{3, 4}]24162125
{4, 4}]545403950
{2, 5}]148525
{3, 5}]75885200
{4, 5}]5048036025
{5, 5}]114678709000
{2, 6}]29350
{3, 6}]110273275
{4, 6}]22945154050
{5, 6}]1231494256550
{6, 6}]27995704239850
{2, 7}]1475
{3, 7}]75885200
{4, 7}]55531376500
{5, 7}]7175800860250
{6, 7}]334030085380350
{7, 7}]7584889119913750
{3, 8}]24162125
{4, 8}]74278763500
{5, 8}]24352783493100
{6, 8}]2329042266808650
{7, 8}]97887416945961075
{8, 8}]2218998811196105750
{3, 9}]3270050
{4, 9}]55531376500
{5, 9}]50034381769600
{6, 9}]10084936612321850
{7, 9}]782114760930236000
{8, 9}]30429684503634827875
{9, 9}]688579463588598857500
{3, 10}]148525
{4, 10}]22945154050
{5, 10}]63477362571125
{6, 10}]28126794522576400
{7, 10}]4075722566708421875
{8, 10}]270605922599775866950
{9, 10}]9910287533252141060075
{10, 10}]223872593965525056524000
{3, 11}]650
{4, 11}]5048036025
{5, 11}]50034381769600
{6, 11}]51642034298930775
{7, 11}]14322131205924119500
{8, 11}]1632070561204989561850
{9, 11}]96088214450066089180650
{10, 11}]3351508924925685769008400
{11, 11}]75590773394298108275641400
{4, 12}]545403950
{5, 12}]24352783493100
{6, 12}]63157566038079800
{7, 12}]34680269311023701250
{8, 12}]6879784715166845894000
{9, 12}]652460665889917943662000
{10, 12}]34897260129076709170702250
{11, 12}]1169273852253720661047855850
{12, 12}]26334146932509192721297606250
{4, 13}]24162125
{5, 13}]7175800860250
{6, 13}]51642034298930775
{7, 13}]58660895139129344250
{8, 13}]20691735554891324819375
{9, 13}]3187856349624109686861750
{10, 13}]261422628471008778452895000
{11, 13}]12925735995730366743674988500
{12, 13}]418749190393922926454264339775
{13, 13}]9418685010993246523213147309050
{4, 14}]250550
{5, 14}]1231494256550
{6, 14}]28126794522576400
{7, 14}]69837157468295256300
{8, 14}]45029496161343522802000
{9, 14}]11425471345666372778573625
{10, 14}]1443695931340763707228964750
{11, 14}]105192221331381719953056030200
{12, 14}]4871005171529900672353774747800
{13, 14}]153346515556322207530993642061375
{14, 14}]3445063666410127667138401567917450
{4, 15}]50
{5, 15}]114678709000
{6, 15}]10084936612321850
{7, 15}]58660895139129344250
{8, 15}]71553701937328489430500
{9, 15}]30455096636986392995454400
{10, 15}]5983442985255839039237107500
{11, 15}]644225116339930387252675093800
{12, 15}]42551462569251226858792953023050
{13, 15}]1863829015771384379547064210671650
{14, 15}]57245804146829441141855075686421600
{15, 15}]1284701496853760180092631899781959250
{5, 16}]5048036025
{6, 16}]2329042266808650
{7, 16}]34680269311023701250
{8, 16}]83451873384004446556500
{9, 16}]60960783194314781836252175
{10, 16}]18858521597882017598430587450
{11, 16}]3018482957837620078514600231550
{12, 16}]284748690462403703849327898236400
{13, 16}]17311291067627079301898110530922200
{14, 16}]722903234302220208838481980961898100
{15, 16}]21731435735419411130551512688193970350
{16, 16}]487219827311876979652523699533587321150
{5, 17}]75885200
{6, 17}]334030085380350
{7, 17}]14322131205924119500
{8, 17}]71553701937328489430500
{9, 17}]92220396289894438953276250
{10, 17}]45641749489863534673387285075
{11, 17}]10956684127545224855242712323800
{12, 17}]1482101901841193380170774085390975
{13, 17}]125101067315642934987038992528141500
{14, 17}]7084069788870929694102349973792379125
{15, 17}]283802089997587090105839672112883654150
{5, 18}]148525
{6, 18}]27995704239850
{7, 18}]4075722566708421875
{8, 18}]45029496161343522802000
{9, 18}]105822944845470819411145650
{10, 18}]85415237718946312165876907100
{11, 18}]31105645711336079302777239697100
{12, 18}]6071452882998806212881647096382400
{13, 18}]713360358445986060308899284173421250
{14, 18}]54760100433813765734980222782145239000
{6, 19}]1231494256550
{7, 19}]782114760930236000
{8, 19}]20691735554891324819375
{9, 19}]92220396289894438953276250
{10, 19}]124182064589288217124451139225
{11, 19}]69561055478912921075310779919000
{12, 19}]19755724290719957639765719857823000
{13, 19}]3245572721974319554949303862415944250
{6, 20}]22945154050
{7, 20}]97887416945961075
{8, 20}]6879784715166845894000
{9, 20}]60960783194314781836252175
{10, 20}]140638929443068626672454410250
{11, 20}]123171917767680954127111199469800
{12, 20}]51423738528601615934359979687767300
{6, 21}]110273275
{7, 21}]7584889119913750
{8, 21}]1632070561204989561850
{9, 21}]30455096636986392995454400
{10, 21}]124182064589288217124451139225
{11, 21}]173303334724056406174320632632850
{6, 22}]29350
{7, 22}]334030085380350
{8, 22}]270605922599775866950
{9, 22}]11425471345666372778573625
{10, 22}]85415237718946312165876907100
{7, 23}]7175800860250
{8, 23}]30429684503634827875
{9, 23}]3187856349624109686861750
{7, 24}]55531376500
{8, 24}]2218998811196105750
{7, 25}]75885200
}
}
\end{adjustbox}
\vskip10pt
\capt{5in}{tab:Instanton_Numbers_2_52}{The genus~0 instanton numbers of total degree $\leqslant 32$ for the family \eqref{eq:CICY_2_52}. The numbers not in this list are either zero, or given by those in the table after a permutation indices.}
\end{table}
BABA BOOEY

==> First_Genus_0_Tables.tex <==
why no work
\begin{table}[p]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{4},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{4},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{4},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/6/.style={select equal part entry of={3}{4},column type = {|l},column name=\hfil $\bm p$},
display columns/7/.style={select equal part entry of={3}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{0, 0, 0, 0, 0, 1}]10
{0, 0, 0, 0, 1, 0}]12
{0, 0, 0, 0, 1, 1}]12
{0, 0, 0, 1, 1, 0}]1
{0, 0, 0, 1, 1, 1}]22
{0, 0, 0, 1, 1, 2}]1
{0, 0, 1, 1, 1, 1}]56
{0, 0, 1, 1, 1, 2}]56
{0, 0, 1, 1, 2, 1}]1
{0, 0, 1, 1, 2, 2}]22
{0, 0, 1, 1, 2, 3}]1
{0, 0, 1, 2, 2, 2}]12
{0, 0, 1, 2, 2, 3}]12
{0, 0, 2, 2, 2, 2}]10
{0, 0, 2, 2, 2, 3}]60
{0, 0, 2, 2, 2, 4}]10
{0, 0, 2, 2, 3, 3}]12
{0, 0, 2, 2, 3, 4}]12
{0, 0, 2, 3, 3, 3}]1
{0, 0, 2, 3, 3, 4}]22
{0, 0, 2, 3, 3, 5}]1
{0, 0, 3, 3, 3, 4}]56
{0, 0, 3, 3, 3, 5}]56
{0, 0, 3, 3, 4, 4}]1
{0, 0, 3, 3, 4, 5}]22
{0, 1, 1, 1, 1, 1}]174
{0, 1, 1, 1, 1, 2}]756
{0, 1, 1, 1, 1, 3}]174
{0, 1, 1, 1, 2, 1}]12
{0, 1, 1, 1, 2, 2}]540
{0, 1, 1, 1, 2, 3}]540
{0, 1, 1, 1, 2, 4}]12
{0, 1, 1, 1, 3, 1}]-2
{0, 1, 1, 1, 3, 2}]10
{0, 1, 1, 1, 3, 3}]96
{0, 1, 1, 1, 3, 4}]10
{0, 1, 1, 1, 3, 5}]-2
{0, 1, 1, 2, 2, 2}]474
{0, 1, 1, 2, 2, 3}]1852
{0, 1, 1, 2, 2, 4}]474
{0, 1, 1, 2, 3, 2}]12
{0, 1, 1, 2, 3, 3}]540
{0, 1, 1, 2, 3, 4}]540
{0, 1, 1, 2, 3, 5}]12
{0, 1, 1, 2, 4, 3}]1
{0, 1, 1, 2, 4, 4}]22
{0, 1, 1, 2, 4, 5}]1
{0, 1, 1, 3, 3, 3}]174
{0, 1, 1, 3, 3, 4}]756
{0, 1, 1, 3, 3, 5}]174
{0, 1, 1, 3, 4, 4}]56
{0, 1, 1, 3, 4, 5}]56
{0, 1, 1, 4, 4, 4}]1
{0, 1, 1, 4, 4, 5}]22
{0, 1, 2, 2, 2, 2}]540
{0, 1, 2, 2, 2, 3}]6708
{0, 1, 2, 2, 2, 4}]6708
{0, 1, 2, 2, 2, 5}]540
{0, 1, 2, 2, 3, 2}]22
{0, 1, 2, 2, 3, 3}]2796
{0, 1, 2, 2, 3, 4}]8860
{0, 1, 2, 2, 3, 5}]2796
{0, 1, 2, 2, 3, 6}]22
{0, 1, 2, 2, 4, 3}]56
{0, 1, 2, 2, 4, 4}]1344
{0, 1, 2, 2, 4, 5}]1344
{0, 1, 2, 2, 4, 6}]56
{0, 1, 2, 2, 5, 4}]1
{0, 1, 2, 2, 5, 5}]22
{0, 1, 2, 3, 3, 3}]1344
{0, 1, 2, 3, 3, 4}]13968
{0, 1, 2, 3, 3, 5}]13968
{0, 1, 2, 3, 3, 6}]1344
{0, 1, 2, 3, 4, 3}]22
{0, 1, 2, 3, 4, 4}]2796
{0, 1, 2, 3, 4, 5}]8860
{0, 1, 2, 3, 5, 4}]12
{0, 1, 2, 4, 4, 4}]540
{0, 1, 3, 3, 3, 3}]798
{0, 1, 3, 3, 3, 4}]25662
{0, 1, 3, 3, 3, 5}]69528
{0, 1, 3, 3, 4, 3}]12
{0, 1, 3, 3, 4, 4}]6708
{0, 2, 2, 2, 2, 2}]756
{0, 2, 2, 2, 2, 3}]25662
{0, 2, 2, 2, 2, 4}]69516
{0, 2, 2, 2, 2, 5}]25662
{0, 2, 2, 2, 2, 6}]756
{0, 2, 2, 2, 3, 2}]56
{0, 2, 2, 2, 3, 3}]13968
{0, 2, 2, 2, 3, 4}]103000
{0, 2, 2, 2, 3, 5}]103000
{0, 2, 2, 2, 3, 6}]13968
{0, 2, 2, 2, 4, 3}]756
{0, 2, 2, 2, 4, 4}]25662
{0, 2, 2, 2, 4, 5}]69516
{0, 2, 2, 2, 5, 4}]540
{0, 2, 2, 3, 3, 2}]1
{0, 2, 2, 3, 3, 3}]8860
{0, 2, 2, 3, 3, 4}]176251
{0, 2, 2, 3, 3, 5}]425712
{0, 2, 2, 3, 4, 3}]540
{0, 2, 2, 3, 4, 4}]54504
{0, 2, 2, 4, 4, 3}]10
{0, 2, 3, 3, 3, 3}]6708
{0, 2, 3, 3, 3, 4}]342924
{0, 2, 3, 3, 4, 3}]474
{0, 3, 3, 3, 3, 3}]6204
{1, 1, 1, 1, 1, 1}]700
{1, 1, 1, 1, 1, 2}]8900
{1, 1, 1, 1, 1, 3}]8900
{1, 1, 1, 1, 1, 4}]700
{1, 1, 1, 1, 2, 1}]66
{1, 1, 1, 1, 2, 2}]8892
{1, 1, 1, 1, 2, 3}]27492
{1, 1, 1, 1, 2, 4}]8892
{1, 1, 1, 1, 2, 5}]66
{1, 1, 1, 1, 3, 1}]-24
{1, 1, 1, 1, 3, 2}]180
{1, 1, 1, 1, 3, 3}]9444
{1, 1, 1, 1, 3, 4}]9444
{1, 1, 1, 1, 3, 5}]180
{1, 1, 1, 1, 3, 6}]-24
{1, 1, 1, 1, 4, 1}]3
{1, 1, 1, 1, 4, 2}]-22
{1, 1, 1, 1, 4, 3}]59
{1, 1, 1, 1, 4, 4}]1024
{1, 1, 1, 1, 4, 5}]59
{1, 1, 1, 1, 4, 6}]-22
{1, 1, 1, 1, 4, 7}]3
{1, 1, 1, 2, 2, 2}]10792
{1, 1, 1, 2, 2, 3}]95648
{1, 1, 1, 2, 2, 4}]95648
{1, 1, 1, 2, 2, 5}]10792
{1, 1, 1, 2, 3, 2}]276
{1, 1, 1, 2, 3, 3}]43326
{1, 1, 1, 2, 3, 4}]125676
{1, 1, 1, 2, 3, 5}]43326
{1, 1, 1, 2, 3, 6}]276
{1, 1, 1, 2, 4, 2}]-48
{1, 1, 1, 2, 4, 3}]432
{1, 1, 1, 2, 4, 4}]22320
{1, 1, 1, 2, 4, 5}]22320
{1, 1, 1, 2, 4, 6}]432
{1, 1, 1, 2, 5, 2}]3
{1, 1, 1, 2, 5, 3}]-22
{1, 1, 1, 2, 5, 4}]59
{1, 1, 1, 2, 5, 5}]1024
{1, 1, 1, 3, 3, 3}]22680
{1, 1, 1, 3, 3, 4}]194664
{1, 1, 1, 3, 3, 5}]194664
{1, 1, 1, 3, 3, 6}]22680
{1, 1, 1, 3, 4, 3}]276
{1, 1, 1, 3, 4, 4}]43326
{1, 1, 1, 3, 4, 5}]125676
{1, 1, 1, 3, 5, 3}]-24
{1, 1, 1, 3, 5, 4}]180
{1, 1, 1, 4, 4, 4}]10792
{1, 1, 2, 2, 2, 2}]15902
{1, 1, 2, 2, 2, 3}]369646
{1, 1, 2, 2, 2, 4}]920760
{1, 1, 2, 2, 2, 5}]369646
{1, 1, 2, 2, 2, 6}]15902
{1, 1, 2, 2, 3, 2}]596
{1, 1, 2, 2, 3, 3}]210748
{1, 1, 2, 2, 3, 4}]1399712
{1, 1, 2, 2, 3, 5}]1399712
{1, 1, 2, 2, 3, 6}]210748
{1, 1, 2, 2, 4, 2}]-176
{1, 1, 2, 2, 4, 3}]3558
{1, 1, 2, 2, 4, 4}]360222
{1, 1, 2, 2, 4, 5}]964648
{1, 1, 2, 2, 5, 2}]36
{1, 1, 2, 2, 5, 3}]-400
{1, 1, 2, 2, 5, 4}]2560
{1, 1, 2, 2, 6, 2}]-4
{1, 1, 2, 2, 6, 3}]30
{1, 1, 2, 3, 3, 2}]2
{1, 1, 2, 3, 3, 3}]139918
{1, 1, 2, 3, 3, 4}]2449206
{1, 1, 2, 3, 3, 5}]5705460
{1, 1, 2, 3, 4, 3}]2676
{1, 1, 2, 3, 4, 4}]766084
{1, 1, 2, 3, 5, 3}]-376
{1, 1, 2, 4, 4, 3}]20
{1, 1, 3, 3, 3, 3}]112196
{1, 1, 3, 3, 3, 4}]4878540
{1, 1, 3, 3, 4, 3}]2775
{1, 2, 2, 2, 2, 2}]27600
{1, 2, 2, 2, 2, 3}]1585020
{1, 2, 2, 2, 2, 4}]8537376
{1, 2, 2, 2, 2, 5}]8537376
{1, 2, 2, 2, 2, 6}]1585020
{1, 2, 2, 2, 3, 2}]1344
{1, 2, 2, 2, 3, 3}]1097052
{1, 2, 2, 2, 3, 4}]14667648
{1, 2, 2, 2, 3, 5}]32044488
{1, 2, 2, 2, 4, 2}]-552
{1, 2, 2, 2, 4, 3}]26364
{1, 2, 2, 2, 4, 4}]4907940
{1, 2, 2, 2, 5, 2}]198
{1, 2, 2, 2, 5, 3}]-3960
{1, 2, 2, 2, 6, 2}]-48
{1, 2, 2, 3, 3, 2}]24
{1, 2, 2, 3, 3, 3}]878696
{1, 2, 2, 3, 3, 4}]28577520
{1, 2, 2, 3, 4, 2}]-2
{1, 2, 2, 3, 4, 3}]24120
{1, 2, 3, 3, 3, 3}]823008
{2, 2, 2, 2, 2, 2}]52740
{2, 2, 2, 2, 2, 3}]7545520
{2, 2, 2, 2, 2, 4}]80109420
{2, 2, 2, 2, 2, 5}]166265920
{2, 2, 2, 2, 3, 2}]2928
{2, 2, 2, 2, 3, 3}]6157524
{2, 2, 2, 2, 3, 4}]154063572
{2, 2, 2, 2, 4, 2}]-1338
{2, 2, 2, 2, 4, 3}]178908
{2, 2, 2, 2, 5, 2}]660
{2, 2, 2, 3, 3, 2}]142
{2, 2, 2, 3, 3, 3}]5734779
{2, 2, 2, 3, 4, 2}]-24
}
}
\end{adjustbox}
\vskip10pt
\capt{5in}{tab:Instanton_Numbers_6_36}{The genus~0 instanton numbers of total degree $\leqslant 15$ for the family \eqref{eq:CICY_6_36}. The numbers not in this list are either zero, or given by those in the table after a permutation of the first five indices. The sixth index \textbf{cannot} be exchanged with the others.}
\end{table}
\begin{table}[p]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{3},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{0, 0, 0, 0, 0, 0, 1}]10
{0, 0, 0, 0, 1, 0, 0}]6
{0, 0, 0, 0, 1, 0, 1}]6
{0, 0, 0, 0, 1, 1, 1}]6
{0, 0, 0, 1, 1, 0, 1}]1
{0, 0, 0, 1, 1, 1, 1}]20
{0, 0, 0, 1, 1, 1, 2}]1
{0, 0, 1, 1, 1, 1, 1}]28
{0, 0, 1, 1, 1, 1, 2}]28
{0, 0, 1, 1, 1, 2, 2}]28
{0, 0, 1, 1, 2, 1, 2}]1
{0, 0, 1, 1, 2, 2, 2}]20
{0, 0, 1, 1, 2, 2, 3}]1
{0, 0, 1, 2, 2, 2, 2}]6
{0, 0, 1, 2, 2, 2, 3}]6
{0, 0, 1, 2, 2, 3, 3}]6
{0, 0, 2, 2, 2, 2, 3}]10
{0, 0, 2, 2, 2, 3, 3}]40
{0, 0, 2, 2, 2, 3, 4}]10
{0, 0, 2, 2, 3, 3, 3}]6
{0, 1, 1, 1, 1, 1, 1}]24
{0, 1, 1, 1, 1, 1, 2}]126
{0, 1, 1, 1, 1, 1, 3}]24
{0, 1, 1, 1, 1, 2, 2}]504
{0, 1, 1, 1, 1, 2, 3}]126
{0, 1, 1, 1, 1, 3, 3}]24
{0, 1, 1, 1, 2, 1, 2}]6
{0, 1, 1, 1, 2, 1, 3}]6
{0, 1, 1, 1, 2, 2, 2}]264
{0, 1, 1, 1, 2, 2, 3}]264
{0, 1, 1, 1, 2, 2, 4}]6
{0, 1, 1, 1, 2, 3, 3}]264
{0, 1, 1, 1, 2, 3, 4}]6
{0, 1, 1, 1, 3, 1, 3}]-2
{0, 1, 1, 1, 3, 2, 3}]10
{0, 1, 1, 1, 3, 3, 3}]80
{0, 1, 1, 1, 3, 3, 4}]10
{0, 1, 1, 2, 2, 2, 2}]72
{0, 1, 1, 2, 2, 2, 3}]330
{0, 1, 1, 2, 2, 2, 4}]72
{0, 1, 1, 2, 2, 3, 3}]1192
{0, 1, 1, 2, 2, 3, 4}]330
{0, 1, 1, 2, 3, 2, 3}]6
{0, 1, 1, 2, 3, 2, 4}]6
{0, 1, 1, 2, 3, 3, 3}]264
{0, 1, 2, 2, 2, 2, 2}]6
{0, 1, 2, 2, 2, 2, 3}]264
{0, 1, 2, 2, 2, 2, 4}]264
{0, 1, 2, 2, 2, 3, 3}]3090
{0, 1, 2, 2, 3, 2, 3}]1
{0, 2, 2, 2, 2, 2, 3}]126
{1, 1, 1, 1, 1, 1, 1}]20
{1, 1, 1, 1, 1, 1, 2}]330
{1, 1, 1, 1, 1, 1, 3}]330
{1, 1, 1, 1, 1, 1, 4}]20
{1, 1, 1, 1, 1, 2, 2}]4120
{1, 1, 1, 1, 1, 2, 3}]4120
{1, 1, 1, 1, 1, 2, 4}]330
{1, 1, 1, 1, 1, 3, 3}]4120
{1, 1, 1, 1, 1, 3, 4}]330
{1, 1, 1, 1, 1, 4, 4}]20
{1, 1, 1, 1, 2, 1, 2}]15
{1, 1, 1, 1, 2, 1, 3}]36
{1, 1, 1, 1, 2, 1, 4}]15
{1, 1, 1, 1, 2, 2, 2}]1692
{1, 1, 1, 1, 2, 2, 3}]5478
{1, 1, 1, 1, 2, 2, 4}]1692
{1, 1, 1, 1, 2, 2, 5}]15
{1, 1, 1, 1, 2, 3, 3}]16464
{1, 1, 1, 1, 2, 3, 4}]5478
{1, 1, 1, 1, 3, 1, 3}]-12
{1, 1, 1, 1, 3, 1, 4}]-12
{1, 1, 1, 1, 3, 2, 3}]90
{1, 1, 1, 1, 3, 2, 4}]90
{1, 1, 1, 1, 3, 3, 3}]4644
{1, 1, 1, 1, 4, 1, 4}]3
{1, 1, 1, 2, 2, 2, 2}]480
{1, 1, 1, 2, 2, 2, 3}]4916
{1, 1, 1, 2, 2, 2, 4}]4916
{1, 1, 1, 2, 2, 3, 3}]42908
{1, 1, 1, 2, 3, 2, 3}]54
{1, 1, 2, 2, 2, 2, 2}]80
{1, 1, 2, 2, 2, 2, 3}]3293
{1, 2, 2, 2, 2, 2, 2}]6
}
}
\end{adjustbox}
\vskip10pt
\capt{5in}{tab:Instanton_Numbers_7_27}{The genus~0 instanton numbers of total degree $\leqslant 13$ for the family \eqref{eq:CICY_7_27}. The numbers not in this list are either zero, or given by those in the table after a permutations of the first five and last two indices. The sixth and seventh indices \textbf{cannot} be exchanged with the first five.}
\end{table}
\begin{table}[p]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{3},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{1, 0, 0, 0}]48
{1, 1, 0, 0}]160
{1, 1, 1, 0}]2432
{1, 1, 1, 1}]86016
{2, 1, 0, 0}]48
{2, 1, 1, 0}]5056
{2, 1, 1, 1}]518784
{2, 2, 0, 0}]128
{2, 2, 1, 0}]34640
{2, 2, 1, 1}]7037184
{2, 2, 2, 0}]507904
{2, 2, 2, 1}]171165840
{2, 2, 2, 2}]6547900416
{3, 1, 1, 0}]2432
{3, 1, 1, 1}]899072
{3, 2, 0, 0}]48
{3, 2, 1, 0}]61824
{3, 2, 1, 1}]28639616
{3, 2, 2, 0}]2089008
{3, 2, 2, 1}]1297013760
{3, 2, 2, 2}]80605022416
{3, 3, 0, 0}]160
{3, 3, 1, 0}]308352
{3, 3, 1, 1}]241754112
{3, 3, 2, 0}]17677056
{3, 3, 2, 1}]17200647552
{3, 3, 2, 2}]1557963029504
{3, 3, 3, 0}]252810752
{3, 3, 3, 1}]352652451840
{3, 3, 3, 2}]43431181213824
{3, 3, 3, 3}]1646607181615104
{4, 1, 1, 0}]160
{4, 1, 1, 1}]518784
{4, 2, 1, 0}]34640
{4, 2, 1, 1}]44662400
{4, 2, 2, 0}]3265280
{4, 2, 2, 1}]4042603552
{4, 2, 2, 2}]426305384448
{4, 3, 0, 0}]48
{4, 3, 1, 0}]508160
{4, 3, 1, 1}]789382400
{4, 3, 2, 0}]57521568
{4, 3, 2, 1}]94371041920
{4, 3, 2, 2}]13002686858864
{4, 3, 3, 0}]1424625024
{4, 3, 3, 1}]3031512413312
{4, 3, 3, 2}]527889850255360
{4, 3, 3, 3}]27526058324060160
{4, 4, 0, 0}]128
{4, 4, 1, 0}]2089008
{4, 4, 1, 1}]4985888864
{4, 4, 2, 0}]360824832
{4, 4, 2, 1}]871452197440
{4, 4, 2, 2}]166647022068736
{4, 4, 3, 0}]13391051328
{4, 4, 3, 1}]39844405855232
{4, 4, 3, 2}]9199812356321968
{4, 4, 3, 3}]627205272329861504
{4, 4, 4, 0}]188051928064
{4, 4, 4, 1}]741058165634496
{4, 4, 4, 2}]217057048330727424
{4, 4, 4, 3}]18647281489625577504
{4, 4, 4, 4}]699794636853614635008
{5, 1, 1, 1}]86016
{5, 2, 1, 0}]5056
{5, 2, 1, 1}]28639616
{5, 2, 2, 0}]2089008
{5, 2, 2, 1}]5834714624
{5, 2, 2, 2}]1108729141920
{5, 3, 1, 0}]308352
{5, 3, 1, 1}]1154723840
{5, 3, 2, 0}]84056832
{5, 3, 2, 1}]249714336000
{5, 3, 2, 2}]54663940002816
{5, 3, 3, 0}]3808483584
{5, 3, 3, 1}]12944311033856
{5, 3, 3, 2}]3295227059205504
{5, 3, 3, 3}]240139807447941120
{5, 4, 0, 0}]48
{5, 4, 1, 0}]3265984
{5, 4, 1, 1}]14129065088
{5, 4, 2, 0}]1017784976
{5, 4, 2, 1}]3874428076928
{5, 4, 2, 2}]1074177329475184
{5, 4, 3, 0}]59821118208
{5, 4, 3, 1}]260287936814720
{5, 4, 3, 2}]82385600163793920
{5, 4, 3, 3}]7471070109015318656
{5, 4, 4, 0}]1268723299376
{5, 4, 4, 1}]6894039650704512
{5, 4, 4, 2}]2643331064630855200
{5, 4, 4, 3}]291051848701788699648
{5, 4, 4, 4}]13862614815470765167056
{5, 5, 0, 0}]160
{5, 5, 1, 0}]11746432
{5, 5, 1, 1}]73320878080
{5, 5, 2, 0}]5243776704
{5, 5, 2, 1}]27965750549248
{5, 5, 2, 2}]10380731579151872
{5, 5, 3, 0}]432161466624
{5, 5, 3, 1}]2545321829650432
{5, 5, 3, 2}]1042877238127097984
{5, 5, 3, 3}]120304302520611954688
{5, 5, 4, 0}]12709250594240
{5, 5, 4, 1}]90222224188616064
{5, 5, 4, 2}]43400958203031979648
{5, 5, 4, 3}]5917889244182186813696
{5, 5, 4, 4}]347399539693965379619648
{5, 5, 5, 0}]176223512332928
{5, 5, 5, 1}]1575672398623395840
{5, 5, 5, 2}]922075476759511908864
{5, 5, 5, 3}]151692725887218685190144
{5, 5, 5, 4}]10726096697730587601447552
{5, 5, 5, 5}]399456970261757309912334336
{6, 1, 1, 1}]2432
{6, 2, 1, 0}]48
{6, 2, 1, 1}]7037184
{6, 2, 2, 0}]507904
{6, 2, 2, 1}]4042603552
{6, 2, 2, 2}]1514352078848
{6, 3, 1, 0}]61824
{6, 3, 1, 1}]789382400
{6, 3, 2, 0}]57521568
{6, 3, 2, 1}]342823329792
{6, 3, 2, 2}]125771915722896
{6, 3, 3, 0}]5243776704
{6, 3, 3, 1}]30008993843584
{6, 3, 3, 2}]11575415612576768
{6, 3, 3, 3}]1203234568961692800
{6, 4, 1, 0}]2089008
{6, 4, 1, 1}]19804670208
{6, 4, 2, 0}]1424616960
{6, 4, 2, 1}]9173232641616
{6, 4, 2, 2}]3846287763468288
{6, 4, 3, 0}]141793830384
{6, 4, 3, 1}]938779827042688
{6, 4, 3, 2}]419700792333851408
{6, 4, 3, 3}]51546803704385918976
{6, 4, 4, 0}]4650991239168
{6, 4, 4, 1}]35938232545114592
{6, 4, 4, 2}]18502170216819978240
{6, 4, 4, 3}]2653048822718080612368
{6, 4, 4, 4}]161629518930438998396928
{6, 5, 0, 0}]48
{6, 5, 1, 0}]17677056
{6, 5, 1, 1}]188011416064
{6, 5, 2, 0}]13391051328
{6, 5, 2, 1}]107087122937856
{6, 5, 2, 2}]55530466229981712
{6, 5, 3, 0}]1651763971584
{6, 5, 3, 1}]13704006681994624
{6, 5, 3, 2}]7493044028521115648
{6, 5, 3, 3}]1120675249090550046720
{6, 5, 4, 0}]69188204803344
{6, 5, 4, 1}]661446106005076224
{6, 5, 4, 2}]409473371380697240000
{6, 5, 4, 3}]70283944963932592401152
{6, 5, 4, 4}]5129348718881933358532960
{6, 5, 5, 0}]1335543626995200
{6, 5, 5, 1}]15470217373819587584
{6, 5, 5, 2}]11284911987863253245440
{6, 5, 5, 3}]2276112606495732006202112
{6, 5, 5, 4}]195588673772290431107673344
{6, 6, 0, 0}]128
{6, 6, 1, 0}]57521568
{6, 6, 1, 1}]845112783616
{6, 6, 2, 0}]59821080576
{6, 6, 2, 1}]645375311627376
{6, 6, 2, 2}]435566317842866176
{6, 6, 3, 0}]9911375239392
{6, 6, 3, 1}]108118212077621248
{6, 6, 3, 2}]74937314945510009952
{6, 6, 3, 3}]13961655375523769282816
{6, 6, 4, 0}]549828820220928
{6, 6, 4, 1}]6736033668350881952
{6, 6, 4, 2}]5160552306598346379264
{6, 6, 4, 3}]1080443741007758375555472
{6, 6, 4, 4}]95469681182710628821921792
{6, 6, 5, 0}]13962620228584512
{6, 6, 5, 1}]201987366061445211648
{6, 6, 5, 2}]178213464042928851755872
{6, 6, 5, 3}]42979893686208656793686016
{6, 6, 6, 0}]191827050005069824
{6, 6, 6, 1}]3375664486259351631456
{6, 6, 6, 2}]3521325683147770386726912
{7, 2, 1, 1}]518784
{7, 2, 2, 0}]34640
{7, 2, 2, 1}]1297013760
{7, 2, 2, 2}]1108729141920
{7, 3, 1, 0}]2432
{7, 3, 1, 1}]241754112
{7, 3, 2, 0}]17677056
{7, 3, 2, 1}]249714336000
{7, 3, 2, 2}]165296580806656
{7, 3, 3, 0}]3808483584
{7, 3, 3, 1}]39529406119936
{7, 3, 3, 2}]24136954745543808
{7, 3, 3, 3}]3672469607846903808
{7, 4, 1, 0}]508160
{7, 4, 1, 1}]14129065088
{7, 4, 2, 0}]1017784976
{7, 4, 2, 1}]12163074768640
{7, 4, 2, 2}]8102781267426048
{7, 4, 3, 0}]188051992832
{7, 4, 3, 1}]1984799528343552
{7, 4, 3, 2}]1294128535920058368
{7, 4, 3, 3}]219681085367035373952
{7, 4, 4, 0}]9911375239392
{7, 4, 4, 1}]112338620588205056
{7, 4, 4, 2}]79594696896349282688
{7, 4, 4, 3}]15110868372965862621696
{7, 4, 4, 4}]1189045428745766422260768
{7, 5, 1, 0}]11746432
{7, 5, 1, 1}]255547666432
{7, 5, 2, 0}]18178255616
{7, 5, 2, 1}]233839970568832
{7, 5, 2, 2}]176514847485662208
{7, 5, 3, 0}]3600925105536
{7, 5, 3, 1}]43715576259518464
{7, 5, 3, 2}]32805238780261668736
{7, 5, 3, 3}]6480417642541472432128
{7, 5, 4, 0}]221844802863872
{7, 5, 4, 1}]2932079676057142912
{7, 5, 4, 2}]2387966888748874810112
{7, 5, 4, 3}]523912487781610422477568
{7, 5, 4, 4}]47981652609161486365088768
{7, 5, 5, 0}]6036801603750144
{7, 5, 5, 1}]92621472022310780928
{7, 5, 5, 2}]85897234681261670146944
{7, 5, 5, 3}]21540883712581909578244096
{7, 6, 0, 0}]48
{7, 6, 1, 0}]84056832
{7, 6, 1, 1}]2010040031104
{7, 6, 2, 0}]141793830384
}
}
\end{adjustbox}
\vskip10pt
\capt{5in}{tab:Instanton_Numbers_4_68}{The genus~0 instanton numbers of total degree $\leqslant 20$ for the family \eqref{eq:CICY_4_68}. The numbers not in this list are either zero, or given by those in the table after a permutation indices.}
\end{table}
\begin{table}[p]\notag
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{3},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{7, 6, 2, 1}]2208595900084224
{7, 6, 2, 2}]2021884379122016048
{7, 6, 3, 0}]33789217322496
{7, 6, 3, 1}]503495581721955456
{7, 6, 3, 2}]455218569908331757568
{7, 6, 3, 3}]107719074363142059583360
{7, 6, 4, 0}]2566483940906640
{7, 6, 4, 1}]41379145350412949504
{7, 6, 4, 2}]40123559676936131346720
{7, 6, 4, 3}]10410193126310745548984320
{7, 6, 5, 0}]87046894784712960
{7, 6, 5, 1}]1607540052866407577728
{7, 6, 5, 2}]1749693070862210564431872
{7, 6, 6, 0}]1576912001012723760
{7, 6, 6, 1}]34462954830661856456704
{7, 7, 0, 0}]160
{7, 7, 1, 0}]252810752
{7, 7, 1, 1}]8087692763136
{7, 7, 2, 0}]567589415680
{7, 7, 2, 1}]11584959011321216
{7, 7, 2, 2}]13491384176760961024
{7, 7, 3, 0}]176223512332928
{7, 7, 3, 1}]3369477175185817600
{7, 7, 3, 2}]3792683314958877584384
{7, 7, 3, 3}]1099277650161884440166400
{7, 7, 4, 0}]17175761255142144
{7, 7, 4, 1}]348295401563531685632
{7, 7, 4, 2}]412395106599944043177984
{7, 7, 5, 0}]740932627227834624
{7, 7, 5, 1}]16875996286670980751360
{7, 7, 6, 0}]16999688846773790208
{8, 2, 1, 1}]5056
{8, 2, 2, 0}]128
{8, 2, 2, 1}]171165840
{8, 2, 2, 2}]426305384448
{8, 3, 1, 1}]28639616
{8, 3, 2, 0}]2089008
{8, 3, 2, 1}]94371041920
{8, 3, 2, 2}]125771915722896
{8, 3, 3, 0}]1424625024
{8, 3, 3, 1}]30008993843584
{8, 3, 3, 2}]30743146145765888
{8, 3, 3, 3}]7079306295276204288
{8, 4, 1, 0}]34640
{8, 4, 1, 1}]4985888864
{8, 4, 2, 0}]360824832
{8, 4, 2, 1}]9173232641616
{8, 4, 2, 2}]10353839703716352
{8, 4, 3, 0}]141793830384
{8, 4, 3, 1}]2538964516666880
{8, 4, 3, 2}]2508525839463392816
{8, 4, 3, 3}]602927912105481193728
{8, 4, 4, 0}]12709250181888
{8, 4, 4, 1}]219342311907269104
{8, 4, 4, 2}]219737543096535650304
{8, 4, 4, 3}]56255611905947864806512
{8, 4, 4, 4}]5785403639953201842686976
{8, 5, 1, 0}]3265984
{8, 5, 1, 1}]188011416064
{8, 5, 2, 0}]13391051328
{8, 5, 2, 1}]302207140853120
{8, 5, 2, 2}]347926332689829040
{8, 5, 3, 0}]4650991497216
{8, 5, 3, 1}]86320414207198848
{8, 5, 3, 2}]91592941667768938752
{8, 5, 3, 3}]24378159414883707592448
{8, 5, 4, 0}]439063136203008
{8, 5, 4, 1}]8247835975441925056
{8, 5, 4, 2}]9033581369124138593840
{8, 5, 4, 3}]2573204027887680476759296
{8, 5, 5, 0}]17175761255142144
{8, 5, 5, 1}]356496506323192211328
{8, 5, 5, 2}]428090722447387987896384
{8, 6, 1, 0}]57521568
{8, 6, 1, 1}]2668638725632
{8, 6, 2, 0}]188051928064
{8, 6, 2, 1}]4533354437642480
{8, 6, 2, 2}]5860852677002366976
{8, 6, 3, 0}]69188204803344
{8, 6, 3, 1}]1462074329960965376
{8, 6, 3, 2}]1771264367116721723008
{8, 6, 3, 3}]542307422558027394152960
{8, 6, 4, 0}]7456149925576704
{8, 6, 4, 1}]162132923614385349360
{8, 6, 4, 2}]203054957441346394726912
{8, 6, 5, 0}]343945562331791376
{8, 6, 5, 1}]8263402711793164324608
{8, 6, 6, 0}]8277365987776740864
{8, 7, 0, 0}]48
{8, 7, 1, 0}]360828928
{8, 7, 1, 1}]18129723322752
{8, 7, 2, 0}]1268723299376
{8, 7, 2, 1}]36298079877646592
{8, 7, 2, 2}]55987725237356145792
{8, 7, 3, 0}]549828822442752
{8, 7, 3, 1}]14005384303898305024
{8, 7, 3, 2}]20171041734451334944000
{8, 7, 4, 0}]71290241748070896
{8, 7, 4, 1}]1864208769268632504064
{8, 7, 5, 0}]3988612138839842816
{8, 8, 0, 0}]128
{8, 8, 1, 0}]1017784976
{8, 8, 1, 1}]66748924807328
{8, 8, 2, 0}]4650991239168
{8, 8, 2, 1}]170418886235419696
{8, 8, 2, 2}]328173467451404489600
{8, 8, 3, 0}]2566483940906640
{8, 8, 3, 1}]82211057906371385344
{8, 8, 4, 0}]417176124089319424
{9, 2, 2, 1}]7037184
{9, 2, 2, 2}]80605022416
{9, 3, 1, 1}]899072
{9, 3, 2, 0}]61824
{9, 3, 2, 1}]17200647552
{9, 3, 2, 2}]54663940002816
{9, 3, 3, 0}]252810752
{9, 3, 3, 1}]12944311033856
{9, 3, 3, 2}]24136954745543808
{9, 3, 3, 3}]8791828001566988288
{9, 4, 1, 0}]160
{9, 4, 1, 1}]789382400
{9, 4, 2, 0}]57521568
{9, 4, 2, 1}]3874428076928
{9, 4, 2, 2}]8102781267426048
{9, 4, 3, 0}]59821118208
{9, 4, 3, 1}]1984799528343552
{9, 4, 3, 2}]3120841582270747392
{9, 4, 3, 3}]1094190143621388343680
{9, 4, 4, 0}]9911375239392
{9, 4, 4, 1}]273504607073902144
{9, 4, 4, 2}]400065629964453039984
{9, 4, 4, 3}]141106319957374906048512
{9, 5, 1, 0}]308352
{9, 5, 1, 1}]73320878080
{9, 5, 2, 0}]5243776704
{9, 5, 2, 1}]233839970568832
{9, 5, 2, 2}]435172594319284224
{9, 5, 3, 0}]3600925105536
{9, 5, 3, 1}]108024514779267072
{9, 5, 3, 2}]167816512674800089472
{9, 5, 3, 3}]61564588462323994361856
{9, 5, 4, 0}]549828822442752
{9, 5, 4, 1}]15172240325024688384
{9, 5, 4, 2}]22894439058514947334656
{9, 5, 5, 0}]31786723861681536
{9, 5, 5, 1}]913426712060194627584
{9, 6, 1, 0}]17677056
{9, 6, 1, 1}]2010040031104
{9, 6, 2, 0}]141793830384
{9, 6, 2, 1}]5744002412760576
{9, 6, 2, 2}]10966073503132221968
{9, 6, 3, 0}]87594475420800
{9, 6, 3, 1}]2738079662657568640
{9, 6, 3, 2}]4572692498129982156800
{9, 6, 4, 0}]13962620228584512
{9, 6, 4, 1}]420332107728557286912
{9, 6, 5, 0}]895919580397273344
{9, 7, 1, 0}]252810752
{9, 7, 1, 1}]23624438407168
{9, 7, 2, 0}]1651763971584
{9, 7, 2, 1}]70930323016569984
{9, 7, 2, 2}]150750588373893541888
{9, 7, 3, 0}]1071736381056384
{9, 7, 3, 1}]37743466871928029184
{9, 7, 4, 0}]191827050036601856
{9, 8, 0, 0}]48
{9, 8, 1, 0}]1424625024
{9, 8, 1, 1}]142582803775232
{9, 8, 2, 0}]9911375239392
{9, 8, 2, 1}]497106580728095936
{9, 8, 3, 0}]7456149932740608
{9, 9, 0, 0}]160
{9, 9, 1, 0}]3808483584
{9, 9, 1, 1}]487860526727168
{9, 9, 2, 0}]33789217322496
{10, 2, 2, 1}]34640
{10, 2, 2, 2}]6547900416
{10, 3, 1, 1}]2432
{10, 3, 2, 0}]48
{10, 3, 2, 1}]1297013760
{10, 3, 2, 2}]13002686858864
{10, 3, 3, 0}]17677056
{10, 3, 3, 1}]3031512413312
{10, 3, 3, 2}]11575415612576768
{10, 3, 3, 3}]7079306295276204288
{10, 4, 1, 1}]44662400
{10, 4, 2, 0}]3265280
{10, 4, 2, 1}]871452197440
{10, 4, 2, 2}]3846287763468288
{10, 4, 3, 0}]13391051328
{10, 4, 3, 1}]938779827042688
{10, 4, 3, 2}]2508525839463392816
{10, 4, 3, 3}]1332539766738727936000
{10, 4, 4, 0}]4650991239168
{10, 4, 4, 1}]219342311907269104
{10, 4, 4, 2}]487713798985291233280
{10, 5, 1, 0}]5056
{10, 5, 1, 1}]14129065088
{10, 5, 2, 0}]1017784976
{10, 5, 2, 1}]107087122937856
{10, 5, 2, 2}]347926332689829040
{10, 5, 3, 0}]1651763971584
{10, 5, 3, 1}]86320414207198848
{10, 5, 3, 2}]204999947699695388672
{10, 5, 4, 0}]439063136203008
{10, 5, 4, 1}]18557339208009894656
{10, 5, 5, 0}]38952597058723520
{10, 6, 1, 0}]2089008
{10, 6, 1, 1}]845112783616
{10, 6, 2, 0}]59821080576
{10, 6, 2, 1}]4533354437642480
{10, 6, 2, 2}]13486794785676976128
{10, 6, 3, 0}]69188204803344
{10, 6, 3, 1}]3368380766765580288
{10, 6, 4, 0}]17175761244601344
{10, 7, 1, 0}]84056832
{10, 7, 1, 1}]18129723322752
{10, 7, 2, 0}]1268723299376
{10, 7, 2, 1}]88462669038163968
{10, 7, 3, 0}]1335543626995200
{10, 8, 1, 0}]1017784976
{10, 8, 1, 1}]182970871579264
{10, 8, 2, 0}]12709250181888
{10, 9, 0, 0}]48
{10, 9, 1, 0}]5243776704
{10, 10, 0, 0}]128
{11, 2, 2, 2}]171165840
{11, 3, 2, 1}]28639616
{11, 3, 2, 2}]1557963029504
{11, 3, 3, 0}]308352
{11, 3, 3, 1}]352652451840
{11, 3, 3, 2}]3295227059205504
{11, 3, 3, 3}]3672469607846903808
{11, 4, 1, 1}]518784
}
}
\end{adjustbox}
\vskip10pt
\caption*{\tref{tab:Instanton_Numbers_4_68} continued.}
\end{table}
\begin{table}[p]\notag
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{3},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{11, 4, 2, 0}]34640
{11, 4, 2, 1}]94371041920
{11, 4, 2, 2}]1074177329475184
{11, 4, 3, 0}]1424625024
{11, 4, 3, 1}]260287936814720
{11, 4, 3, 2}]1294128535920058368
{11, 4, 4, 0}]1268723299376
{11, 4, 4, 1}]112338620588205056
{11, 5, 1, 1}]1154723840
{11, 5, 2, 0}]84056832
{11, 5, 2, 1}]27965750549248
{11, 5, 2, 2}]176514847485662208
{11, 5, 3, 0}]432161466624
{11, 5, 3, 1}]43715576259518464
{11, 5, 4, 0}]221844802863872
{11, 6, 1, 0}]61824
{11, 6, 1, 1}]188011416064
{11, 6, 2, 0}]13391051328
{11, 6, 2, 1}]2208595900084224
{11, 6, 3, 0}]33789217322496
{11, 7, 1, 0}]11746432
{11, 7, 1, 1}]8087692763136
{11, 7, 2, 0}]567589415680
{11, 8, 1, 0}]360828928
{12, 2, 2, 2}]507904
{12, 3, 2, 1}]61824
{12, 3, 2, 2}]80605022416
{12, 3, 3, 0}]160
{12, 3, 3, 1}]17200647552
{12, 3, 3, 2}]527889850255360
{12, 4, 1, 1}]160
{12, 4, 2, 1}]4042603552
{12, 4, 2, 2}]166647022068736
{12, 4, 3, 0}]57521568
{12, 4, 3, 1}]39844405855232
{12, 4, 4, 0}]188051928064
{12, 5, 1, 1}]28639616
{12, 5, 2, 0}]2089008
{12, 5, 2, 1}]3874428076928
{12, 5, 3, 0}]59821118208
{12, 6, 1, 0}]48
{12, 6, 1, 1}]19804670208
{12, 6, 2, 0}]1424616960
{12, 7, 1, 0}]508160
{13, 3, 2, 2}]1297013760
{13, 3, 3, 1}]241754112
{13, 4, 2, 1}]44662400
{13, 4, 3, 0}]508160
{13, 5, 1, 1}]86016
{13, 5, 2, 0}]5056
}
}
\end{adjustbox}
\vskip10pt
\caption*{\tref{tab:Instanton_Numbers_4_68} continued.}
\end{table}
\begin{table}[p]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{3},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{3},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{3},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B
{0, 1}]50
{1, 1}]650
{1, 2}]1475
{2, 2}]29350
{1, 3}]650
{2, 3}]148525
{3, 3}]3270050
{1, 4}]50
{2, 4}]250550
{3, 4}]24162125
{4, 4}]545403950
{2, 5}]148525
{3, 5}]75885200
{4, 5}]5048036025
{5, 5}]114678709000
{2, 6}]29350
{3, 6}]110273275
{4, 6}]22945154050
{5, 6}]1231494256550
{6, 6}]27995704239850
{2, 7}]1475
{3, 7}]75885200
{4, 7}]55531376500
{5, 7}]7175800860250
{6, 7}]334030085380350
{7, 7}]7584889119913750
{3, 8}]24162125
{4, 8}]74278763500
{5, 8}]24352783493100
{6, 8}]2329042266808650
{7, 8}]97887416945961075
{8, 8}]2218998811196105750
{3, 9}]3270050
{4, 9}]55531376500
{5, 9}]50034381769600
{6, 9}]10084936612321850
{7, 9}]782114760930236000
{8, 9}]30429684503634827875
{9, 9}]688579463588598857500
{3, 10}]148525
{4, 10}]22945154050
{5, 10}]63477362571125
{6, 10}]28126794522576400
{7, 10}]4075722566708421875
{8, 10}]270605922599775866950
{9, 10}]9910287533252141060075
{10, 10}]223872593965525056524000
{3, 11}]650
{4, 11}]5048036025
{5, 11}]50034381769600
{6, 11}]51642034298930775
{7, 11}]14322131205924119500
{8, 11}]1632070561204989561850
{9, 11}]96088214450066089180650
{10, 11}]3351508924925685769008400
{11, 11}]75590773394298108275641400
{4, 12}]545403950
{5, 12}]24352783493100
{6, 12}]63157566038079800
{7, 12}]34680269311023701250
{8, 12}]6879784715166845894000
{9, 12}]652460665889917943662000
{10, 12}]34897260129076709170702250
{11, 12}]1169273852253720661047855850
{12, 12}]26334146932509192721297606250
{4, 13}]24162125
{5, 13}]7175800860250
{6, 13}]51642034298930775
{7, 13}]58660895139129344250
{8, 13}]20691735554891324819375
{9, 13}]3187856349624109686861750
{10, 13}]261422628471008778452895000
{11, 13}]12925735995730366743674988500
{12, 13}]418749190393922926454264339775
{13, 13}]9418685010993246523213147309050
{4, 14}]250550
{5, 14}]1231494256550
{6, 14}]28126794522576400
{7, 14}]69837157468295256300
{8, 14}]45029496161343522802000
{9, 14}]11425471345666372778573625
{10, 14}]1443695931340763707228964750
{11, 14}]105192221331381719953056030200
{12, 14}]4871005171529900672353774747800
{13, 14}]153346515556322207530993642061375
{14, 14}]3445063666410127667138401567917450
{4, 15}]50
{5, 15}]114678709000
{6, 15}]10084936612321850
{7, 15}]58660895139129344250
{8, 15}]71553701937328489430500
{9, 15}]30455096636986392995454400
{10, 15}]5983442985255839039237107500
{11, 15}]644225116339930387252675093800
{12, 15}]42551462569251226858792953023050
{13, 15}]1863829015771384379547064210671650
{14, 15}]57245804146829441141855075686421600
{15, 15}]1284701496853760180092631899781959250
{5, 16}]5048036025
{6, 16}]2329042266808650
{7, 16}]34680269311023701250
{8, 16}]83451873384004446556500
{9, 16}]60960783194314781836252175
{10, 16}]18858521597882017598430587450
{11, 16}]3018482957837620078514600231550
{12, 16}]284748690462403703849327898236400
{13, 16}]17311291067627079301898110530922200
{14, 16}]722903234302220208838481980961898100
{15, 16}]21731435735419411130551512688193970350
{16, 16}]487219827311876979652523699533587321150
{5, 17}]75885200
{6, 17}]334030085380350
{7, 17}]14322131205924119500
{8, 17}]71553701937328489430500
{9, 17}]92220396289894438953276250
{10, 17}]45641749489863534673387285075
{11, 17}]10956684127545224855242712323800
{12, 17}]1482101901841193380170774085390975
{13, 17}]125101067315642934987038992528141500
{14, 17}]7084069788870929694102349973792379125
{15, 17}]283802089997587090105839672112883654150
{5, 18}]148525
{6, 18}]27995704239850
{7, 18}]4075722566708421875
{8, 18}]45029496161343522802000
{9, 18}]105822944845470819411145650
{10, 18}]85415237718946312165876907100
{11, 18}]31105645711336079302777239697100
{12, 18}]6071452882998806212881647096382400
{13, 18}]713360358445986060308899284173421250
{14, 18}]54760100433813765734980222782145239000
{6, 19}]1231494256550
{7, 19}]782114760930236000
{8, 19}]20691735554891324819375
{9, 19}]92220396289894438953276250
{10, 19}]124182064589288217124451139225
{11, 19}]69561055478912921075310779919000
{12, 19}]19755724290719957639765719857823000
{13, 19}]3245572721974319554949303862415944250
{6, 20}]22945154050
{7, 20}]97887416945961075
{8, 20}]6879784715166845894000
{9, 20}]60960783194314781836252175
{10, 20}]140638929443068626672454410250
{11, 20}]123171917767680954127111199469800
{12, 20}]51423738528601615934359979687767300
{6, 21}]110273275
{7, 21}]7584889119913750
{8, 21}]1632070561204989561850
{9, 21}]30455096636986392995454400
{10, 21}]124182064589288217124451139225
{11, 21}]173303334724056406174320632632850
{6, 22}]29350
{7, 22}]334030085380350
{8, 22}]270605922599775866950
{9, 22}]11425471345666372778573625
{10, 22}]85415237718946312165876907100
{7, 23}]7175800860250
{8, 23}]30429684503634827875
{9, 23}]3187856349624109686861750
{7, 24}]55531376500
{8, 24}]2218998811196105750
{7, 25}]75885200
}
}
\end{adjustbox}
\vskip10pt
\capt{5in}{tab:Instanton_Numbers_2_52}{The genus~0 instanton numbers of total degree $\leqslant 32$ for the family \eqref{eq:CICY_2_52}. The numbers not in this list are either zero, or given by those in the table after a permutation indices.}
\end{table}
BABA BOOEY

==> basics.tex <==
%!TEX root=../main.tex

\chapter{Some Essentials}
I know not where I am.

==> chapter1.tex <==
%!TEX root=../main.tex

\chapter{Flux Compactifications}

\epigraph{Rose: I can’t even touch it. Seems to be in a state of flux.\\
Donna: What does that mean?\\
Rose: I don’t know.}{Russell T Davies, \textit{Turn Left}}




==> prisoner636.tex <==
\begin{adjustbox}{width=\columnwidth,center}
\tiny{\pgfplotstabletypeset[
col sep=space,
white space chars={]},
ignore chars={\ },
every head row/.style={before row=\hline,after row=\hline\hline},
every first row/.style={before row=\vrule height12pt width0pt depth0pt},
every last row/.style={before row=\vrule height0pt width0pt depth6pt,after row=\hline},
%after row=\hline,    %  Uncomment this to get back lines between all rows.
columns={A,B,A,B,A,B,A,B},
display columns/0/.style={select equal part entry of={0}{4},column type = {|l},column name=\vrule height12pt width0pt depth6pt \hfil $\bm p$},
display columns/1/.style={select equal part entry of={0}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/2/.style={select equal part entry of={1}{4},column type = {|l},column name=\hfil $\bm p$},
display columns/3/.style={select equal part entry of={1}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/4/.style={select equal part entry of={2}{4},column type = {|l},column name=\hfil $\bm p$},
display columns/5/.style={select equal part entry of={2}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
display columns/6/.style={select equal part entry of={3}{4},column type = {|l},column name=\hfil $\bm p$},
display columns/7/.style={select equal part entry of={3}{4},column type = {|l|},column name=\hfil $n^{(0)}_{\bm p}$},
string type]
{
A ] B

{0, 0, 0, 0, 0, 1}]10
{0, 0, 0, 0, 1, 0}]12
{0, 0, 0, 0, 1, 1}]12
{0, 0, 0, 1, 1, 0}]1
{0, 0, 0, 1, 1, 1}]22
{0, 0, 0, 1, 1, 2}]1
{0, 0, 1, 1, 1, 1}]56
{0, 0, 1, 1, 1, 2}]56
{0, 0, 1, 1, 2, 1}]1
{0, 0, 1, 1, 2, 2}]22
{0, 0, 1, 1, 2, 3}]1
{0, 0, 1, 2, 2, 2}]12
{0, 0, 1, 2, 2, 3}]12
{0, 0, 2, 2, 2, 2}]10
{0, 0, 2, 2, 2, 3}]60
{0, 0, 2, 2, 2, 4}]10
{0, 0, 2, 2, 3, 3}]12
{0, 0, 2, 2, 3, 4}]12
{0, 0, 2, 3, 3, 3}]1
{0, 0, 2, 3, 3, 4}]22
{0, 0, 2, 3, 3, 5}]1
{0, 0, 3, 3, 3, 4}]56
{0, 0, 3, 3, 3, 5}]56
{0, 0, 3, 3, 4, 4}]1
{0, 0, 3, 3, 4, 5}]22
{0, 1, 1, 1, 1, 1}]174
{0, 1, 1, 1, 1, 2}]756
{0, 1, 1, 1, 1, 3}]174
{0, 1, 1, 1, 2, 1}]12
{0, 1, 1, 1, 2, 2}]540
{0, 1, 1, 1, 2, 3}]540
{0, 1, 1, 1, 2, 4}]12
{0, 1, 1, 1, 3, 1}]-2
{0, 1, 1, 1, 3, 2}]10
{0, 1, 1, 1, 3, 3}]96
{0, 1, 1, 1, 3, 4}]10
{0, 1, 1, 1, 3, 5}]-2
{0, 1, 1, 2, 2, 2}]474
{0, 1, 1, 2, 2, 3}]1852
{0, 1, 1, 2, 2, 4}]474
{0, 1, 1, 2, 3, 2}]12
{0, 1, 1, 2, 3, 3}]540
{0, 1, 1, 2, 3, 4}]540
{0, 1, 1, 2, 3, 5}]12
{0, 1, 1, 2, 4, 3}]1
{0, 1, 1, 2, 4, 4}]22
{0, 1, 1, 2, 4, 5}]1
{0, 1, 1, 3, 3, 3}]174
{0, 1, 1, 3, 3, 4}]756
{0, 1, 1, 3, 3, 5}]174
{0, 1, 1, 3, 4, 4}]56
{0, 1, 1, 3, 4, 5}]56
{0, 1, 1, 4, 4, 4}]1
{0, 1, 1, 4, 4, 5}]22
{0, 1, 2, 2, 2, 2}]540
{0, 1, 2, 2, 2, 3}]6708
{0, 1, 2, 2, 2, 4}]6708
{0, 1, 2, 2, 2, 5}]540
{0, 1, 2, 2, 3, 2}]22
{0, 1, 2, 2, 3, 3}]2796
{0, 1, 2, 2, 3, 4}]8860
{0, 1, 2, 2, 3, 5}]2796
{0, 1, 2, 2, 3, 6}]22
{0, 1, 2, 2, 4, 3}]56
{0, 1, 2, 2, 4, 4}]1344
{0, 1, 2, 2, 4, 5}]1344
{0, 1, 2, 2, 4, 6}]56
{0, 1, 2, 2, 5, 4}]1
{0, 1, 2, 2, 5, 5}]22
{0, 1, 2, 3, 3, 3}]1344
{0, 1, 2, 3, 3, 4}]13968
{0, 1, 2, 3, 3, 5}]13968
{0, 1, 2, 3, 3, 6}]1344
{0, 1, 2, 3, 4, 3}]22
{0, 1, 2, 3, 4, 4}]2796
{0, 1, 2, 3, 4, 5}]8860
{0, 1, 2, 3, 5, 4}]12
{0, 1, 2, 4, 4, 4}]540
{0, 1, 3, 3, 3, 3}]798
{0, 1, 3, 3, 3, 4}]25662
{0, 1, 3, 3, 3, 5}]69528
{0, 1, 3, 3, 4, 3}]12
{0, 1, 3, 3, 4, 4}]6708
{0, 2, 2, 2, 2, 2}]756
{0, 2, 2, 2, 2, 3}]25662
{0, 2, 2, 2, 2, 4}]69516
{0, 2, 2, 2, 2, 5}]25662
{0, 2, 2, 2, 2, 6}]756
{0, 2, 2, 2, 3, 2}]56
{0, 2, 2, 2, 3, 3}]13968
{0, 2, 2, 2, 3, 4}]103000
{0, 2, 2, 2, 3, 5}]103000
{0, 2, 2, 2, 3, 6}]13968
{0, 2, 2, 2, 4, 3}]756
{0, 2, 2, 2, 4, 4}]25662
{0, 2, 2, 2, 4, 5}]69516
{0, 2, 2, 2, 5, 4}]540
{0, 2, 2, 3, 3, 2}]1
{0, 2, 2, 3, 3, 3}]8860
{0, 2, 2, 3, 3, 4}]176251
{0, 2, 2, 3, 3, 5}]425712
{0, 2, 2, 3, 4, 3}]540
{0, 2, 2, 3, 4, 4}]54504
{0, 2, 2, 4, 4, 3}]10
{0, 2, 3, 3, 3, 3}]6708
{0, 2, 3, 3, 3, 4}]342924
{0, 2, 3, 3, 4, 3}]474
{0, 3, 3, 3, 3, 3}]6204
{1, 1, 1, 1, 1, 1}]700
{1, 1, 1, 1, 1, 2}]8900
{1, 1, 1, 1, 1, 3}]8900
{1, 1, 1, 1, 1, 4}]700
{1, 1, 1, 1, 2, 1}]66
{1, 1, 1, 1, 2, 2}]8892
{1, 1, 1, 1, 2, 3}]27492
{1, 1, 1, 1, 2, 4}]8892
{1, 1, 1, 1, 2, 5}]66
{1, 1, 1, 1, 3, 1}]-24
{1, 1, 1, 1, 3, 2}]180
{1, 1, 1, 1, 3, 3}]9444
{1, 1, 1, 1, 3, 4}]9444
{1, 1, 1, 1, 3, 5}]180
{1, 1, 1, 1, 3, 6}]-24
{1, 1, 1, 1, 4, 1}]3
{1, 1, 1, 1, 4, 2}]-22
{1, 1, 1, 1, 4, 3}]59
{1, 1, 1, 1, 4, 4}]1024
{1, 1, 1, 1, 4, 5}]59
{1, 1, 1, 1, 4, 6}]-22
{1, 1, 1, 1, 4, 7}]3
{1, 1, 1, 2, 2, 2}]10792
{1, 1, 1, 2, 2, 3}]95648
{1, 1, 1, 2, 2, 4}]95648
{1, 1, 1, 2, 2, 5}]10792
{1, 1, 1, 2, 3, 2}]276
{1, 1, 1, 2, 3, 3}]43326
{1, 1, 1, 2, 3, 4}]125676
{1, 1, 1, 2, 3, 5}]43326
{1, 1, 1, 2, 3, 6}]276
{1, 1, 1, 2, 4, 2}]-48
{1, 1, 1, 2, 4, 3}]432
{1, 1, 1, 2, 4, 4}]22320
{1, 1, 1, 2, 4, 5}]22320
{1, 1, 1, 2, 4, 6}]432
{1, 1, 1, 2, 5, 2}]3
{1, 1, 1, 2, 5, 3}]-22
{1, 1, 1, 2, 5, 4}]59
{1, 1, 1, 2, 5, 5}]1024
{1, 1, 1, 3, 3, 3}]22680
{1, 1, 1, 3, 3, 4}]194664
{1, 1, 1, 3, 3, 5}]194664
{1, 1, 1, 3, 3, 6}]22680
{1, 1, 1, 3, 4, 3}]276
{1, 1, 1, 3, 4, 4}]43326
{1, 1, 1, 3, 4, 5}]125676
{1, 1, 1, 3, 5, 3}]-24
{1, 1, 1, 3, 5, 4}]180
{1, 1, 1, 4, 4, 4}]10792
{1, 1, 2, 2, 2, 2}]15902
{1, 1, 2, 2, 2, 3}]369646
{1, 1, 2, 2, 2, 4}]920760
{1, 1, 2, 2, 2, 5}]369646
{1, 1, 2, 2, 2, 6}]15902
{1, 1, 2, 2, 3, 2}]596
{1, 1, 2, 2, 3, 3}]210748
{1, 1, 2, 2, 3, 4}]1399712
{1, 1, 2, 2, 3, 5}]1399712
{1, 1, 2, 2, 3, 6}]210748
{1, 1, 2, 2, 4, 2}]-176
{1, 1, 2, 2, 4, 3}]3558
{1, 1, 2, 2, 4, 4}]360222
{1, 1, 2, 2, 4, 5}]964648
{1, 1, 2, 2, 5, 2}]36
{1, 1, 2, 2, 5, 3}]-400
{1, 1, 2, 2, 5, 4}]2560
{1, 1, 2, 2, 6, 2}]-4
{1, 1, 2, 2, 6, 3}]30
{1, 1, 2, 3, 3, 2}]2
{1, 1, 2, 3, 3, 3}]139918
{1, 1, 2, 3, 3, 4}]2449206
{1, 1, 2, 3, 3, 5}]5705460
{1, 1, 2, 3, 4, 3}]2676
{1, 1, 2, 3, 4, 4}]766084
{1, 1, 2, 3, 5, 3}]-376
{1, 1, 2, 4, 4, 3}]20
{1, 1, 3, 3, 3, 3}]112196
{1, 1, 3, 3, 3, 4}]4878540
{1, 1, 3, 3, 4, 3}]2775
{1, 2, 2, 2, 2, 2}]27600
{1, 2, 2, 2, 2, 3}]1585020
{1, 2, 2, 2, 2, 4}]8537376
{1, 2, 2, 2, 2, 5}]8537376
{1, 2, 2, 2, 2, 6}]1585020
{1, 2, 2, 2, 3, 2}]1344
{1, 2, 2, 2, 3, 3}]1097052
{1, 2, 2, 2, 3, 4}]14667648
{1, 2, 2, 2, 3, 5}]32044488
{1, 2, 2, 2, 4, 2}]-552
{1, 2, 2, 2, 4, 3}]26364
{1, 2, 2, 2, 4, 4}]4907940
{1, 2, 2, 2, 5, 2}]198
{1, 2, 2, 2, 5, 3}]-3960
{1, 2, 2, 2, 6, 2}]-48
{1, 2, 2, 3, 3, 2}]24
{1, 2, 2, 3, 3, 3}]878696
{1, 2, 2, 3, 3, 4}]28577520
{1, 2, 2, 3, 4, 2}]-2
{1, 2, 2, 3, 4, 3}]24120
{1, 2, 3, 3, 3, 3}]823008
{2, 2, 2, 2, 2, 2}]52740
{2, 2, 2, 2, 2, 3}]7545520
{2, 2, 2, 2, 2, 4}]80109420
{2, 2, 2, 2, 2, 5}]166265920
{2, 2, 2, 2, 3, 2}]2928
{2, 2, 2, 2, 3, 3}]6157524
{2, 2, 2, 2, 3, 4}]154063572
{2, 2, 2, 2, 4, 2}]-1338
{2, 2, 2, 2, 4, 3}]178908
{2, 2, 2, 2, 5, 2}]660
{2, 2, 2, 3, 3, 2}]142
{2, 2, 2, 3, 3, 3}]5734779
{2, 2, 2, 3, 4, 2}]-24

}
}
\end{adjustbox}
